Distributed Sketching for Randomized Optimization: Exact Characterization, Concentration and Lower Bounds

We consider distributed optimization methods for problems where forming the Hessian is computationally challenging and communication is a significant bottleneck. We leverage randomized sketches for reducing the problem dimensions as well as preserving privacy and improving straggler resilience in asynchronous distributed systems. We derive novel approximation guarantees for classical sketching methods and establish tight concentration results that serve as both upper and lower bounds on the error. We then extend our analysis to the accuracy of parameter averaging for distributed sketches. Furthermore, we develop unbiased parameter averaging methods for randomized second order optimization for regularized problems that employ sketching of the Hessian. Existing works do not take the bias of the estimators into consideration, which limits their application to massively parallel computation. We provide closed-form formulas for regularization parameters and step sizes that provably minimize the bias for sketched Newton directions. Additionally, we demonstrate the implications of our theoretical findings via large scale experiments on a serverless cloud computing platform.

==> highprob_bound_OLD.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
-- UNCOMMENT/DELETE START HERE --
\subsection{High Probability Error Bound via Lipschitz Concentration} \label{subsec:lipschitz}

Let us consider the single-sketch estimator $\hat{x}$.
\begin{align}
    f(\hat{x}) - f(x^*) &= \|A(\hat{x}-x^*)\|_2^2 \nonumber \\
    &= \|A(A^TS^TSA)^{-1}A^TS^TSb^{\perp}\|_2^2 \nonumber \\
    &= \|A(SA)^\dagger Sb^{\perp}\|_2^2
\end{align}
where the superscript $\hspace{-1mm}~^\dagger$ refers to the pseudo-inverse.

\begin{theorem}[Concentration of Lipschitz functions of Gaussian Variables] \label{thm:lipschitz_concentration} [cite]

Let $W \in \mathbb{R}^{m \times n}$ be a matrix with i.i.d. entries $W_{ij} \sim \mathcal{N}(0,1)$. Define $h : \mathbb{R}^{m \times n} \rightarrow \mathbb{R}$ and assume it is $L$-Lipschitz with respect to the Euclidean norm, i.e., $|h(W)-h(W^\prime)| \leq L \|W-W^\prime\|_2$ for all $W,W^\prime \in \mathbb{R}^{m \times n}$. Then,
\begin{align}
    P\left(|h(W)- \Exs[h(W)]| \geq \epsilon \right) \leq 2e^{-\frac{\epsilon^2}{2L^2}} \mbox{ for all } \epsilon \geq 0.
\end{align}
\end{theorem}

We note that $S$ is scaled such that $\Exs[S^TS]=I$. Therefore, its entries are distributed as $\mathcal{N}(0,1/m)$. It follows that the entries of $\sqrt{m}S$ are distributed as $\mathcal{N}(0,1)$.

The vector $Sb^\perp$ is distributed as $\mathcal{N}(0, \|b^\perp\|_2^2/m)$. We scale it by $\sqrt{m} / \|b^\perp\|_2$ to obtain the standard normal distribution. That is, the entries of $\frac{\sqrt{m}}{\|b^\perp\|_2}Sb^\perp$ are distributed as $\mathcal{N}(0,1)$. We note that the distribution of $Sb^\perp$ is the same when conditioned on $SA$ since the columns of $A$ are perpendicular to $b^\perp$, i.e., $A^Tb^\perp=0$.
%
Next, we note that 
\begin{align}
f(\hat{x}) - f(x^*) &= \left\Vert \frac{\|b^\perp\|_2}{\sqrt{m}} A(SA)^\dagger \frac{\sqrt{m}}{\|b^\perp\|_2} Sb^\perp \right\Vert_2^2 
\end{align}
%
Let us define $z := \frac{\sqrt{m}}{\|b^\perp\|_2}Sb^\perp$ and introduce the function
\begin{align}
    g(z) := \left\Vert \frac{\|b^\perp\|_2}{\sqrt{m}} A(SA)^\dagger z\right\Vert_2 .
\end{align}
where $\sqrt{f(\hat{x}) - f(x^*)} = g\left(\frac{\sqrt{m}}{\|b^\perp\|_2}Sb^\perp\right)$.

Next, by Theorem \ref{thm:lipschitz_concentration}, we have 
\begin{align}
    P\left(\left| g(z) - \Exs[g(z)]\right| \geq \epsilon | SA\right) \leq 2e^{-\frac{\epsilon^2}{2L^2}} 
\end{align}
where $L$ is a Lipschitz constant of the function $g(z)$. We can find a Lipschitz constant for $g(z)$ as follows
\begin{align}
    \left| g(z) - g(z^\prime) \right| &= \left| \left\Vert \frac{\|b^\perp\|_2}{\sqrt{m}} A(SA)^\dagger z\right\Vert_2 - \left\Vert \frac{\|b^\perp\|_2}{\sqrt{m}} A(SA)^\dagger z^\prime\right\Vert_2 \right| \nonumber \\
    &= \frac{\|b^\perp\|_2}{\sqrt{m}} \left| \left\Vert A(SA)^\dagger z\right\Vert_2 - \left\Vert A(SA)^\dagger z^\prime\right\Vert_2 \right| \nonumber \\
    &\leq \frac{\|b^\perp\|_2}{\sqrt{m}} \left\Vert A(SA)^\dagger (z-z^\prime) \right\Vert_2
\end{align}
where the inequality in the third line follows from the triangle inequality. We can bound $\|A(SA)^\dagger (z-z^\prime)\|_2$ as follows:
%
\begin{align}
    \|A(SA)^\dagger (z-z^\prime)\|_2 &= \|U\Sigma V^T(SU\Sigma V^T)^\dagger (z-z^\prime)\|_2 \nonumber \\
    &= \|(U^TS^TSU)^{-1}U^TS^T (z-z^\prime)\|_2 \nonumber \\
    &\leq \|(U^TS^TSU)^{-1}U^TS^T \|_2 \|z-z^\prime\|_2 \nonumber \\
    &= \|(SU)^\dagger\|_2 \|z-z^\prime\|_2 \nonumber \\
    &= \frac{1}{\sigma_{\min}(SU)} \|z-z^\prime\|_2 .
\end{align}
%
Hence, we can take $L = \frac{\|b^\perp\|_2}{\sqrt{m}\sigma_{\min}(SU)}$. Plugging this in the result by Theorem 2.4, we obtain
%
\begin{align}
    P\left(\left| g(z) - \Exs[g(z)]\right| \geq \epsilon | SA\right) \leq 2\exp\left(-\frac{m\epsilon^2 \sigma^2_{\min}(SU)}{2\|b^\perp\|_2^2}\right)
\end{align}
%
\mert{We can change save a factor of two in the probability upper bound, i.e., $\exp()$ instead of $2 \exp$ if we only need a one-sided concentration result $g(z)\ge \Exs g(z)+\epsilon$.}
%
Taking the expectation of the above probability gives us
%
\begin{align} \label{eq:exponential_exp}
    P\left(\left| g(z) - \Exs[g(z)]\right| \geq \epsilon \right) &= \Exs\left[P\left(\left| g(z) - \Exs[g(z)]\right| \geq \epsilon | SA\right)\right] \nonumber \\
    &\leq \Exs \left[ 2\exp\left(-\frac{m\epsilon^2 \sigma^2_{\min}(SU)}{2\|b^\perp\|_2^2}\right) \right] \nonumber \\
    &= 2\Exs \left[\exp\left(-\frac{m\epsilon^2 \sigma^2_{\min}(SU)}{2f(x^*)}\right) \right] 
\end{align}
where the first line follows from the law of total probability.
% \mert{We should get the final probability after conditioning on the smallest singular value of $SU$.}


We will use a result for the smallest singular value of the Gaussian matrix $SU$
\begin{align}
    P(\sigma_{\min}(SU) \leq 1 - \sqrt{d/m} - t) \leq \exp(-mt^2/2)
\end{align}
This bound follows from the Lipschitz concentration result in Theorem \ref{thm:lipschitz_concentration} [add citation or write proof for this result?].


Next, we can bound the expression in \eqref{eq:exponential_exp} as follows:
\begin{align}
    &\Exs[\exp(-\gamma \sigma^2_{\min}(SU))] = \nonumber \\
    &=\Exs[e^{-\gamma \sigma^2_{\min}(SU)} | E] P(E) + \Exs[e^{-\gamma \sigma^2_{\min}(SU)} | E^C]P(E^C) \nonumber \\ 
    &\leq e^{-\gamma (1-\sqrt{d/m}-t)^2} (1-e^{-mt^2/2}) + e^{-mt^2/2}
\end{align}
%
where $\gamma := m\epsilon^2 / (2f(x^*))$, which is non-negative and the event $E$ is defined as $\sigma_{\min}(SU) \geq 1-\sqrt{d/m}-t$. 


\begin{align}
    P&\left(\left| \sqrt{f(\hat{x}) - f(x^*)} - \Exs[\sqrt{f(\hat{x}) - f(x^*)}] \right| \geq \epsilon \right) \nonumber \\
    &\leq 2 \left(e^{-\gamma (1-\sqrt{d/m}-t)^2} (1-e^{-mt^2/2}) + e^{-mt^2/2} \right)
\end{align}


We could write the following one-sided concentration result
\begin{align}
    P&\left(\sqrt{f(\hat{x}) - f(x^*)} \geq \Exs[\sqrt{f(\hat{x}) - f(x^*)}] + \epsilon \right) \nonumber \\ 
    &\leq e^{-\gamma (1-\sqrt{d/m}-t)^2} (1-e^{-mt^2/2}) + e^{-mt^2/2}
\end{align}
Squaring the RHS of the inequality inside the probability gives us
\begin{align}
     \Exs&[\sqrt{f(\hat{x}) - f(x^*)}]^2 + \epsilon^2 + 2\epsilon\Exs[\sqrt{f(\hat{x}) - f(x^*)}] \nonumber \\
     & \leq \Exs[f(\hat{x}) - f(x^*)] + \epsilon^2 + 2\epsilon \sqrt{\Exs[f(\hat{x}) - f(x^*)]} \nonumber \\
     &= f(x^*)\frac{d}{m-d-1} + \epsilon^2 + 2\epsilon \sqrt{f(x^*)\frac{d}{m-d-1}}
\end{align}
Note that $\Exs[\sqrt{f(\hat{x}) - f(x^*)}] \leq \sqrt{\Exs[f(\hat{x}) - f(x^*)]}$, which follows from Jensen's inequality for the square root function (which is concave). We have used this relation to obtain the first inequality.
%
Then, the following probability is upper bounded by the same bound
\begin{align}
    P\left( f(\hat{x}) \geq f(x^*)\frac{m-1}{m-d-1} + \epsilon^2 + 2\epsilon \sqrt{f(x^*)\frac{d}{m-d-1}} \right) 
\end{align}



% \mert{Bu Jensen upper-bound'ini kullanarak 
% \begin{align*}  P\left(\sqrt{f(\hat{x}) - f(x^*)} \geq \Exs[\sqrt{f(\hat{x}) - f(x^*)}] + \epsilon \right)\ge\\ P\left(\sqrt{f(\hat{x}) - f(x^*)} \geq \sqrt{\Exs f(\hat{x}) - f(x^*)} + \epsilon \right]\end{align*}
% olarak da yapabiliriz? 
% Daha sonra two-sided Lipschitz concentration ile lower-bound'ini da bulabiliriz belki senin yukaridaki kareyi acarak yaptigin sekilde?
% }
% \burak{Sizin yazdiginiz inequality'de esitsizligin yonunun tersi olmasi lazim sanirim veya yanlis mi dusunuyorum? Lower bound (18)'deki gibi oluyor, belki biraz daha simplify edebiliriz. Upper bound'a da bakacagim.}


% The other one-sided concentration result is
% \begin{align}
%     P&\left(\sqrt{f(\hat{x}) - f(x^*)} \leq \Exs[\sqrt{f(\hat{x}) - f(x^*)}] - \epsilon \right) \nonumber \\ 
%     &\leq e^{-\gamma (1-\sqrt{d/m}-t)^2} (1-e^{-mt^2/2}) + e^{-mt^2/2}
% \end{align}
% ...


\begin{align}
    P&\left( \frac{f(\hat{x})}{f(x^*)} \geq \frac{m-1}{m-d-1} + \frac{\epsilon^2}{f(x^*)} + 2\epsilon \sqrt{\frac{d}{f(x^*)(m-d-1)}} \right) \nonumber \\
    &\leq e^{-\frac{m\epsilon^2}{2f(x^*)} (1-\sqrt{d/m}-t)^2} (1-e^{-mt^2/2}) + e^{-mt^2/2}
\end{align}
%
Making the change of variable $\epsilon \leftarrow 2\sqrt{\frac{df(x^*)}{m-d-1}}\epsilon$ gives us
\begin{align}
    P&\left( \frac{f(\hat{x})}{f(x^*)} \geq \frac{m-1}{m-d-1} + (\epsilon^2+\epsilon)\frac{4d}{m-d-1} \right) \nonumber \\
    &\leq e^{-\frac{2md\epsilon^2}{m-d-1} (1-\sqrt{d/m}-t)^2} (1-e^{-mt^2/2}) + e^{-mt^2/2} 
\end{align}
%
Assuming $\epsilon < 1$, the following bound holds
\begin{align}
    P&\left( \frac{f(\hat{x})}{f(x^*)} \geq \frac{m-1}{m-d-1} + \epsilon \frac{8d}{m-d-1} \right) \nonumber \\
    &\leq e^{-\frac{2md\epsilon^2}{m-d-1} (1-\sqrt{d/m}-t)^2} (1-e^{-mt^2/2}) + e^{-mt^2/2} 
\end{align}
%
Making the change of variable $\epsilon \leftarrow \frac{m-d-1}{8d}$ leads to the bound
\begin{align}
    P&\left( \frac{f(\hat{x})}{f(x^*)} \geq \frac{m-1}{m-d-1} + \epsilon \right) \nonumber \\
    &\leq e^{-\frac{m\epsilon^2(m-d-1)}{32d} (1-\sqrt{d/m}-t)^2} (1-e^{-mt^2/2}) + e^{-mt^2/2} 
\end{align}


\begin{figure}[!t]
\begin{minipage}[b]{1\linewidth}
  \centering
  \centerline{\includegraphics[width=\columnwidth]{src/histogram_and_bound_plot.pdf}}
%   \centerline{(a) }\medskip
\end{minipage}
\caption{This plot shows the probability that optimality ratio is greater than the values shown in the horizontal axis. $t$ is numerically optimized. $n=1000,d=20,m=400$.}
% \label{fig:}
\end{figure}


\noindent \textbf{Averaged Estimator:} Now we consider the averaged estimator $\bar{x}=\frac{1}{q}\sum_{k=1}^q\hat{x}_k$.
\begin{align}
    f(\bar{x}) - f(x^*) &= \|A(\bar{x} - x^*)\|_2^2 \nonumber \\
    &= \left\Vert\frac{1}{q} \sum_{k=1}^q A(A^TS_k^TS_kA)^{-1}A^TS_k^TS_kb^\perp \right\Vert_2^2 \nonumber \\
    &= \left\Vert\frac{1}{q} \sum_{k=1}^q A (S_kA)^\dagger S_kb^\perp \right\Vert_2^2 
\end{align}

Let us define $$g(z_1,\dots,z_q) = \left\Vert\frac{1}{q} \frac{\|b^\perp\|_2}{\sqrt{m}} \sum_{k=1}^q A (S_kA)^\dagger z_k \right\Vert_2$$ where we defined $z_k:=\frac{\sqrt{m}}{\|b^\perp\|_2} S_kb^\perp$, $k=1,\dots,q$. Let us define $$z = \begin{bmatrix} z_1 \\ \vdots \\ z_q \end{bmatrix}$$.

\begin{align}
    &|g(z) - g(z^\prime)| = \frac{\|b^\perp\|_2}{q\sqrt{m}} \left| \left\Vert \sum_{k=1}^q A (S_kA)^\dagger z_k \right\Vert_2 - \left\Vert \sum_{k=1}^q A (S_kA)^\dagger z_k^\prime \right\Vert_2 \right| \nonumber \\
    &\leq \frac{\|b^\perp\|_2}{q\sqrt{m}} \left| \left\Vert \sum_{q=1}^k A(S_kA)^\dagger (z_k - z_k^\prime) \right\Vert_2 \right| \nonumber \\
    &= \frac{\|b^\perp\|_2}{q\sqrt{m}}  \left\Vert \sum_{q=1}^k A(S_kA)^\dagger (z_k - z_k^\prime) \right\Vert_2 \nonumber \\
    &\leq \frac{\|b^\perp\|_2}{q\sqrt{m}} \sum_{q=1}^k \|A(S_kA)^\dagger(z_k-z_k^\prime) \|_2 \nonumber \\
    &= 
\end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{High Probability Error Bound via Gaussian Quadratic Form Concentration}
We recall from the previous subsection that 
\begin{align}
f(\hat{x}) - f(x^*) &= \left\Vert \frac{\|b^\perp\|_2}{\sqrt{m}} A(SA)^\dagger \frac{\sqrt{m}}{\|b^\perp\|_2} Sb^\perp \right\Vert_2^2 
\end{align}
and we define $z := \frac{\sqrt{m}}{\|b^\perp\|_2}Sb^\perp$ and $M := \frac{\|b^\perp\|_2}{\sqrt{m}} A(SA)^\dagger$. This simplifies the previous expression
\begin{align}
    f&(\hat{x}) - f(x^*) = \|Mz\|_2^2 = z^TM^TMz \nonumber \\
    &= z^T \left(\frac{\|b^\perp\|_2^2}{m}{(SA)^\dagger}^TA^TA(SA)^\dagger \right)z \nonumber \\
    &= z^T \left(\frac{\|b^\perp\|_2^2}{m}SA(A^TS^TSA)^{-1}A^TA(A^TS^TSA)^{-1}A^TS^T \right)z \nonumber \\
    &= z^T \left(\frac{\|b^\perp\|_2^2}{m}SU(U^TS^TSU)^{-2}U^TS^T \right)z \nonumber \\
    &= z^T \left(\frac{\|b^\perp\|_2^2}{m} {(SU)^\dagger}^T(SU)^\dagger \right)z
\end{align}
%
We will upper bound the following probabilities
\begin{align}
    P\left(z^TM^TMz > a | SA \right) \mbox{ and } P\left(z^TM^TMz < a | SA \right)
\end{align}
%
First, let us define
%
\begin{align}
    \nu &= 4\|M^TM \|_F^2 = 4 \sum_{j} \sigma_j^2(M^TM) \nonumber \\
    &= 4\frac{\|b^\perp\|_2^4}{m^2} \sum_{j} \sigma_j^4((SU)^\dagger) \nonumber \\
    &\leq 4\frac{\|b^\perp\|_2^4}{m^2} d\sigma^4_{\max}((SU)^\dagger) \nonumber \\
    &= 4\frac{\|b^\perp\|_2^4}{m^2} \frac{d}{\sigma^4_{\min}(SU)}
\end{align}
and similarly, we can lower bound $\nu$ as
\begin{align}
    \nu \geq 4\frac{\|b^\perp\|_2^4}{m^2} d\sigma^4_{\min}((SU)^\dagger) = 4\frac{\|b^\perp\|_2^4}{m^2}\frac{d}{\sigma^4_{\max}(SU)}
\end{align}
and
\begin{align}
    \beta &= \lambda_{\max}(M^TM) = \sigma^2_{\max}(M) \nonumber \\
    &= \sigma^2_{\max}\left(\frac{\|b^\perp\|_2}{\sqrt{m}}(SU)^\dagger \right) \nonumber \\
    &= \frac{\|b^\perp\|_2^2}{m} \frac{1}{\sigma^2_{\min}(SU)}
\end{align}

The quantity $\frac{\nu}{4\beta}$ is bounded between:
\begin{align}
    \frac{d\|b^\perp\|_2^2}{m\sigma^2_{\min}(SU)} \frac{1}{\kappa^4(SU)}\leq \frac{\nu}{4\beta} \leq \frac{d\|b^\perp\|_2^2}{m\sigma^2_{\min}(SU)}
\end{align}

For $\epsilon > 0$, we have, from Theorem 1 of [cite Improved Concentration Bounds for Gaussian
Quadratic Forms],
\begin{align}
    P&\left(f(\hat{x}) - f(x^*) > \Exs[f(\hat{x}) - f(x^*)] + \epsilon |SA \right) \nonumber \\
    &\leq \exp\left(-\frac{1}{2}\frac{\epsilon^2}{\nu} \right) \nonumber \\
    &\leq \exp\left(-\frac{1}{8}\frac{\epsilon^2m^2\sigma^4_{\min}(SU)}{df^2(x^*)} \right)
\end{align}
We can manipulate the expression further to obtain a probability bound for the optimality ratio as follows:
\begin{align}
    P\left(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1} + \epsilon | SA \right) \leq \exp\left(-\frac{1}{8} \epsilon^2m^2d^{-1}\sigma^4_{\min}(SU) \right)
\end{align}
Taking the expectation of both sides with respect to $SA$ yields
\begin{align}
    P&\left(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1} + \epsilon \right) \leq \Exs\left[e^{-\frac{1}{8} \epsilon^2m^2d^{-1}\sigma^4_{\min}(SU)} \right] \nonumber \\
    &\leq e^{-\frac{1}{8} \epsilon^2m^2d^{-1}(1-\sqrt{d/m}-t)^4}(1-e^{-mt^2/2}) + e^{-mt^2/2}
\end{align}
which is true for $0 < \epsilon \leq \frac{\nu}{4\beta}\frac{1}{f(x^*)}$.

\noindent For $\epsilon > \frac{\nu}{4\beta}\frac{1}{f(x^*)}$, we have
\begin{align}
    P&\left(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1} + \epsilon \right) \leq \Exs\left[e^{\frac{d}{8}} e^{-\frac{1}{4}\epsilon m\sigma^2_{\min}(SU)} \right] \nonumber \\
    &\leq e^{\frac{d}{8}-\frac{1}{4}\epsilon m (1-\sqrt{d/m}-t)^2} (1-e^{-mt^2/2}) + e^{\frac{d}{8}-mt^2/2}
\end{align}

% Bringing the pieces together, we obtain
% \begin{align}
%     P&\left(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1} + \epsilon \right) 
% \end{align}



% \burak{Figure 1'e yeni bound'u ekledim. Histogram'i cizerken hata yapmisim, onu duzelttim, yeni bound'da hata yok sanirim. Su an plot consistent gorunuyor.}
% \mert{Super, tesekkurler! Quadratic form concentration'dan lower-bound'da bulabiliyor muyuz? Onu da plot edebiliriz (sol tarafta olan dagilimi yani).}
% \burak{Bulabiliriz sanirim, simdi bakacagim ona. Bulunca plot'a eklerim.}
% \mert{Tamam. Peki bu kullandigimiz yeni concenration boundda $\epsilon$ un ne kadar buyuk olduguna gore iki farkli regime vardi?}
% \burak{Su an ilk regime'de oldugumuzu assume edip yazdim bound'u.}
% \mert{O zaman $\epsilon$'un uzerinde bir bound mi geliyor eq 32'te?}
% \burak{Evet, hangi regime'de oldugumuzu bilmemiz icin $\nu$'nun exact degeri gerekli ama sanirim.}
% \mert{Su an $\epsilon$'un uzerindeki assumption ne, onu da eklermisin eq 32'ten sonra.}
% \burak{$\epsilon \leq \nu / (4\beta f(x^*))$ oluyor assumption, eklerim tabi.}
% \mert{Bunu yazabilmek icin $\nu$'nun lower-bound'ini mi bulmamiz gerek? Frobenius norm'un lower boundunu maximum singular value ile bulabiliriz 27. denklemin ilk satirinda. Sanirim $\nu/\beta\ge 1$ oluyor? } 
% \mert{Diger regime'deki upper-bound'u da eq 32 gibi yazip simplify edebilir misin? Ikisini combine edip tek bound seklinde yazabiliriz. Ayrica lower-boundlara da bu sekilde bakalim.}
% \burak{Tamamdir hocam tesekkurler.}


% \burak{Iki regime'i de figure 1'de plot ettim. $\nu/(4\beta)$ icin upper ve lower bound eq. (30)'da. Iki regime'i concise bir sekilde yazarken, $\epsilon$ icin olan condition'i $\nu/(4\beta)$ cinsinden yazmamiz gerekcek galiba cunku, $\nu$'nun exact degeri $SU$ matrisine bagli. Veya max(prob1, prob2) seklinde yazabiliriz. }


\noindent \textbf{Error upper bound:} 

\noindent For $0 < \epsilon \leq \frac{\nu}{4\beta}\frac{1}{f(x^*)}$, we have
\begin{align}
    P&\left(\frac{f(\hat{x})}{f(x^*)} < \frac{m-1}{m-d-1} - \epsilon \right) \nonumber \\
    &\leq e^{-\frac{1}{8} \epsilon^2m^2d^{-1}(1-\sqrt{d/m}-t)^4}(1-e^{-mt^2/2}) + e^{-mt^2/2}
\end{align}

\noindent For $\epsilon > \frac{\nu}{4\beta}\frac{1}{f(x^*)}$, we have
\begin{align}
    P&\left(\frac{f(\hat{x})}{f(x^*)} < \frac{m-1}{m-d-1} - \epsilon \right) \nonumber \\
    &\leq e^{\frac{d}{8}-\frac{1}{4}\epsilon m (1-\sqrt{d/m}-t)^2} (1-e^{-mt^2/2}) + e^{\frac{d}{8}-mt^2/2}
\end{align}

\begin{figure}[!t]
\begin{minipage}[b]{1\linewidth}
  \centering
  \centerline{\includegraphics[width=\columnwidth]{src/histogram_and_bound_plot_upperbound.pdf}}
%   \centerline{(a) }\medskip
\end{minipage}
\caption{This plot shows the probability that optimality ratio is lower than the values shown in the horizontal axis. $t$ is numerically optimized. $n=1000,d=20,m=400$.}
% \label{fig:}
\end{figure}

% \mert{Super, tesekkurler!Frobenius normu bound ederken nu upperboundin da bir d faktoru olmayacak mi?  }

% \burak{Evet hocam haklisiniz, orda bir hata yapmisim. Plotlari yeniden yaptim, Lipshitz bound'a daha yaklasti simdi.}


% \mert{Peki eq 30'u ve geri kalan herseyi de duzelttik mi? }

% \burak{Evet onlari duzelttim hocam.}

\mert{Bir de soyle bir improvement yapalim: $\nu = 4 \|M^TM\|_F^2 = Tr ((SU)^T(SU))^{-2}$ olmasi lazim, ben hesaplayinca bu sekilde cikti, bir cok cancellation oluyor. O zaman $\mathbb{E} \|M^TM\|_F^2 =\theta_2$ oluyor, closed form olarak biliyoruz. Daha onceden kullandigimiz Wishart inverse second moment bu, eger bir yanlis yapmadiysam. Bunu su sekilde kullanabiliriz: Concentration bound'i (33) veya (34) te apply ettigimizde aslinda $e^{-\frac{\epsilon...}{\nu}}$ gibi bir upper-bound geliyor $SA$'e conditional olarak. Bu probability nin expectation'ini alip uncondition edersek ve Jensen's inequality ile $\Exs e^{-\frac{\epsilon}{\nu}} \le e^{-\frac{\epsilon}{ \Exs \nu}}$ oldugunu kullanirsak, unconditional probability bound'u $e^{-\frac{\epsilon}{\theta_2}}$ gibi daha iyi olmasi lazim. Boyle yaparsak Frobenius norm'u bound ederken $d$ faktorunu gereksiz yere eklememis oluruz.}



\noindent \textbf{Exact calculation of $\nu$:}
\begin{align} \label{eq:exact_calc_nu}
    \nu &= 4\|M^TM \|_F^2 = 4\left\Vert \frac{\|b^\perp\|_2^2}{m} {(SU)^\dagger}^T(SU)^\dagger\right\Vert_F^2 \nonumber \\
    &= 4\frac{\|b^\perp\|_2^4}{m^2} \left\Vert  {(SU)^\dagger}^T(SU)^\dagger \right\Vert_F^2 \nonumber \\
    &= 4\frac{\|b^\perp\|_2^4}{m^2} \left\Vert  SU(U^TS^TSU)^{-2}U^TS^T \right\Vert_F^2 \nonumber \\
    &= 4\frac{\|b^\perp\|_2^4}{m^2} \tr\left(SU(U^TS^TSU)^{-2}U^TS^TSU(U^TS^TSU)^{-2}U^TS^T \right) \nonumber \\
    &= 4\frac{\|b^\perp\|_2^4}{m^2} \tr\left(SU(U^TS^TSU)^{-3}U^TS^T \right) \nonumber \\
    &= 4\frac{\|b^\perp\|_2^4}{m^2} \tr\left((U^TS^TSU)^{-2} \right)
\end{align}

\noindent The quantity $\frac{\nu}{4\beta}$ will have the following expression:
\begin{align}
    \frac{\nu}{4\beta} = \frac{f(x^*)}{m} \sigma^2_{\min}(SU) \tr\left((U^TS^TSU)^{-2} \right)
\end{align}
%
From Theorem 1 of [cite Improved Concentration Bounds for Gaussian Quadratic Forms],
\begin{align}
    P&\left(f(\hat{x}) - f(x^*) > \Exs[f(\hat{x}) - f(x^*)] + \epsilon |SA \right) \nonumber \\
    &\leq \exp\left(-\frac{1}{2}\frac{\epsilon^2}{\nu} \right) \nonumber \\
    &= \exp \left(-\frac{1}{8} \frac{\epsilon^2 m^2}{ f^2(x^*) \tr\left((U^TS^TSU)^{-2}\right)} \right)
\end{align}
%
Scaling the terms inside the probability by $f(x^*)$ and changing $\epsilon \leftarrow \epsilon f(x^*)$ yields
\begin{align}
    P&\left(\frac{f(\hat{x})}{f(x^*)} > 1 + \frac{d}{m-d-1} + \epsilon | SA \right) \nonumber \\
    &\quad\quad\quad\quad\leq \exp \left(-\frac{1}{8} \frac{\epsilon^2 m^2}{ \tr\left((U^TS^TSU)^{-2}\right)} \right)
\end{align}
Taking the expectation of both sides with respect to $SA$ yields
\begin{align}
    P&\left(\frac{f(\hat{x})}{f(x^*)} > 1 + \frac{d}{m-d-1} + \epsilon\right) \leq \Exs\left[e^{-\frac{1}{8} \frac{\epsilon^2 m^2}{ \tr\left((U^TS^TSU)^{-2}\right)}} \right] \nonumber \\
    &\leq 
\end{align}
% \burak{$\Exs[e^{-\frac{c}{x}}]$ fonksiyonu $x > c/2$ icin concave oluyor. Burda $c=\frac{\epsilon^2m^2}{8}$.}



% \burak{Event tanimlayip, conditioning yapabiliriz belki eskisi gibi:}
% \begin{align}
%     \Exs\left[e^{-\frac{1}{8} \frac{\epsilon^2 m^2}{ \tr\left((U^TS^TSU)^{-2}\right)}} \right] &= \Exs\left[e^{-\frac{1}{8} \frac{\epsilon^2 m^2}{ \tr\left((U^TS^TSU)^{-2}\right)}} | E \right]P(E) \nonumber \\
%     &+ \Exs\left[e^{-\frac{1}{8} \frac{\epsilon^2 m^2}{ \tr\left((U^TS^TSU)^{-2}\right)}} | E^C \right]P(E^C)
% \end{align}
% Let us define the event $E$ as $\tr\left((U^TS^TSU)^{-2}\right) > \frac{\epsilon^2m^2}{16}$.



% \mert{eq 33'ten sonra verdigimiz $\epsilon$ range'inde $1/f(x^*)$ faktoru dogru mu? Sanki $f(\hat x)/f(x^*)$ oranina baktigimiz icin $f(x^*)$ cancel olmasi lazim? Ornegin eq 25'e bakarsak, iki tarafi $f(x^*)$ ile bolsek, sag tarafta $f(x^*)$ iceren terim kalmiyor, o yuzden concentration kisminda $f(x^*)$ olmamasi lazim sanirim? }
% \burak{$1/f(x^*)$ faktoru , $\epsilon \leftarrow \epsilon f(x^*)$ change of variable yapinca geldi. }

% \mert{Ama eq 25'te iki tarafi $f(x^*)^2$'a bolersek sag taraftan kayboluyor.}

% \burak{O durumda, $\nu$'nun tanimi degisince, yine ayni sonuc cikacak galiba.}

% \mert{Dogru olabilir dedigin, ama kontrol edelim.}

% \burak{Tamam kontrol ederim tekrar.  $\nu/(4\beta)$ expressioninda $f(x^*)$ var numerator'da, $1/f(x^*)$ faktoru ile o sadelesecek sanirim.}

% \mert{Bunu da duzeltirsek ve $\theta_2$'yi kullanirsak, bir upper-bound bir lower bound state edelim theorem olarak. $\epsilon$'un kucuk oldugu range daha mantikli, cunku mean'e arbitrary yaklasabiliyor. Relative error upper-bound'unu su sekilde verebiliriz:
% $$P \left( \frac{f(\hat x)}{f(x^*)} > 1 + \frac{d}{m-d-1} +\epsilon \right) \le e^{\frac{-\epsilon^2 m^2(...)}{8d}}$$
% when $\epsilon<\frac{d (1+\sqrt{\frac{d}{m}})^2}{m (1-\sqrt{\frac{d}{m}})^4}$
% }
% \mert{Bu yukarida yazdigimda $f(x^*)$ faktoru $\epsilon$ range'inden ve probability'den eksik olabilir, onu ekleyelim.}

% \mert{Ayni sekilde lower-bound'i da su sekilde sadece kucuk $\epsilon$ rangei icin yazalim
% $$P \left( \frac{f(\hat x)}{f(x^*)} < 1 + \frac{d}{m-d-1} -\epsilon \right) \le e^{\frac{d}{8}-\frac{\epsilon^2 m^2(...)}{8d}}$$
% when $\epsilon<\frac{d (1+\sqrt{\frac{d}{m}})^2}{m (1-\sqrt{\frac{d}{m}})^4}$
% }

% \burak{Tamamdir hocam yazarim bu sekilde, tesekkurler.}
% \burak{$\epsilon$ range'ini yazarken, $SU$ random oldugu icin, with high probability gibi bir ifade mi yazmaliyiz? }
% \mert{$SU$'nun minimum eigenvalue'su icin bir conditioning yapiyoruz ya, ona gore eq (30)'daki lower bound'dan kucuk olmasi yetiyor. Oyle degil mi? }

% \burak{$\sigma_{\min}(SU) \leq 1 - \sqrt{d/m}$ conditioning'ini ordan sonra yapiyoruz sanirim? Eq (30)'daki lower bound'dan kucuk olmasi yetiyor evet, ama ordaki $SU$'nun en kucuk singular value'su ile ilgili exact bir sey soyleyebilir miyiz?}

% \mert{$\theta_2$'yi kullanma kismi karisik, haklisin.}

% \mert{Su iki bound'u kullanirsak olmaz mi istedigimiz bound? 
% \begin{align}
%     P(\sigma_{\min}(SU) \leq 1 - \sqrt{d/m} - t) \leq \exp(-mt^2/2)
% \end{align}
% \begin{align}
%     P(\sigma_{\min}(SU) \geq 1 + \sqrt{d/m} + t) \leq \exp(-mt^2/2)
% \end{align}
% Bunlar da Lipschitz concentration bound'undan geliyor $g(S):=\min_{\|z\|_2=1} \frac{1}{\sqrt{m}}\|Sz\|_2$ fonksiyonu $1/\sqrt{m}$-Lipschitz.}

% \burak{$\epsilon$ icin sizin yukarda yazdiginiz gibi bir condition kullaninca, $\epsilon<\frac{d (1+\sqrt{\frac{d}{m}})^2}{m (1-\sqrt{\frac{d}{m}})^4}$, aslinda bu condition'i saglayan ama $\epsilon < \nu/(4\beta)$ condition'ini saglamayan durumlar dusuk probability'de olabilir degil mi?}
% \mert{Bu singular value'larin iyi oldugu event'e condition edince onemi yok ama?}
% \mert{Bir de suradaki quadratic form concentration resultini kullanabiliriz: Proposition 1  \href{https://arxiv.org/pdf/1901.08736.pdf}{https://arxiv.org/pdf/1901.08736.pdf}}


% \begin{align}
%     P&(f(\hat{x}) - f(x^*) - \frac{df(x^*)}{m-d-1} > 2 \|M^TM\|_F \sqrt{\epsilon} + 2\|M^TM\|_2\epsilon | SA) \nonumber \\
%     &\leq e^{-\epsilon}
% \end{align}
% \mert{Evet, aynen bu sekilde. Burada $SA$ uzerinden uncondition edebilir miyiz $\mathbb{E} \|M^TM\|_F$ ile replace ederek?}

% \burak{Trace terimi sanirim yine $e^{-1/x}$ gibi olacak, islemi tam olarak yapmadim ama henuz. Concave olmazsa yine benzer problem olabilir.}

% \mert{Evet ama, probability operatorunun icerisindeki $SA$'e bagli terimlerin expectationini alabilir miyiz?}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Lipschitz Concentration on the Full Sketching Matrix}

% The entries of the matrix $\sqrt{m}S$ are from the i.i.d. standard normal distribution.

% \begin{align}
% f&(\hat{x}) - f(x^*) = \|A(A^TS^TSA)^{-1}A^TS^TSb^{\perp}\|_2^2 \nonumber \\
% &= \|A(A^T(\sqrt{m}S)^T(\sqrt{m}S)A)^{-1}A^T(\sqrt{m}S)^T(\sqrt{m}S)b^{\perp}\|_2^2
% \end{align}

% \noindent Hence, we can replace all $\sqrt{m}S$ terms with $S$ and assume that the entries of $S$ are distributed as i.i.d. standard normal.

% \begin{align}
%     f&(\hat{x}) - f(x^*) = \|U\Sigma V^T(V\Sigma U^TS^TSU\Sigma V^T)^{-1}V\Sigma U^TS^TSb^{\perp}\|_2^2 \nonumber \\
%     &= \|U(U^TS^TSU)^{-1}U^TS^TSb^\perp \|_2^2 \nonumber \\
%     &= \|(U^TS^TSU)^{-1}U^TS^TSb^\perp \|_2^2 = \|(SU)^\dagger Sb^\perp \|_2^2
% \end{align}

% We will find an upper bound for $|g(S) - g(S^\prime)|$, but first we upper bound $g(S) - g(S^\prime)$:
% %
% \begin{align}
%     &g(S) - g(S^\prime) = \|(SU)^\dagger Sb^\perp\|_2 - \|(S^\prime U)^\dagger S^\prime b^\perp\|_2 \nonumber \\
%     &= \|\left((SU)^\dagger - (S^\prime U)^\dagger + (S^\prime U)^\dagger \right)Sb^\perp\|_2 - \|(S^\prime U)^\dagger S^\prime b^\perp\|_2 \nonumber \\
%     &\leq \| \left((SU)^\dagger - (S^\prime U)^\dagger \right)Sb^\perp \|_2 + \|(S^\prime U)^\dagger Sb^\perp\|_2 - \|(S^\prime U)^\dagger S^\prime b^\perp\|_2 \nonumber \\
%     &\leq \| \left((SU)^\dagger - (S^\prime U)^\dagger \right)Sb^\perp \|_2 + \|(S^\prime U)^\dagger (S-S^\prime)b^\perp\|_2 \nonumber \\
%     &\leq \| (SU)^\dagger - (S^\prime U)^\dagger \|_2 \|Sb^\perp\|_2 + \|(S^\prime U)^\dagger\|_2 \|(S-S^\prime)b^\perp\|_2
% \end{align}

% We can upper bound $\| (SU)^\dagger - (S^\prime U)^\dagger \|_F$ using eq 1.5 [cite On the perturbation of the Moore–Penrose inverse of a matrix], assuming $SU$ and $S^\prime U$ are both full rank (rank = $d$):
% %
% \begin{align}
%     \| (SU)^\dagger - (S^\prime U)^\dagger \|_F &\leq \|(SU)^\dagger\|_2 \|(S^\prime U)^\dagger\|_2 \|(S - S^\prime )U\|_F \nonumber \\
%     &= \frac{1}{\sigma_{\min}(SU)\sigma_{\min}(S^\prime U)} \|(S - S^\prime )U\|_F \nonumber \\
%     &\leq \frac{1}{\sigma_{\min}(SU)\sigma_{\min}(S^\prime U)} \|S - S^\prime \|_F \|U\|_F \nonumber \\
%     &= \frac{\sqrt{d}}{\sigma_{\min}(SU)\sigma_{\min}(S^\prime U)} \|S - S^\prime\|_F
% \end{align}
% %
% The upper bound for $g(S) - g(S^\prime)$ is then as follows:
% %
% \begin{align}
%     &g(S) - g(S^\prime) \nonumber \\
%     &\leq \left(\frac{\sqrt{d} \|Sb^\perp\|_2 }{\sigma_{\min}(SU)\sigma_{\min}(S^\prime U)} + \frac{\|b^\perp\|_2}{\sigma_{\min}(S^\prime U)}  \right) \|S - S^\prime\|_F
% \end{align}
% and similarly, for $g(S^\prime) - g(S)$, it is
% %
% \begin{align}
%     &g(S^\prime) - g(S) \nonumber \\
%     &\leq \left(\frac{\sqrt{d} \|S^\prime b^\perp\|_2 }{\sigma_{\min}(SU)\sigma_{\min}(S^\prime U)} + \frac{\|b^\perp\|_2}{\sigma_{\min}(S U)}  \right) \|S - S^\prime\|_F
% \end{align}
% %
% Then, $|g(S^\prime) - g(S)| \leq $


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{align}
%     &|g(S) - g(S^\prime)| = \left| \| A(SA)^\dagger Sb^\perp \|_2 - \| A(S^\prime A)^\dagger S^\prime b^\perp \|_2  \right| \nonumber \\
%     &= \left| \| \left(A(SA)^\dagger - A(S^\prime A)^\dagger + A(S^\prime A)^\dagger \right)Sb^\perp \|_2 - \| A(S^\prime A)^\dagger S^\prime b^\perp \|_2  \right| \nonumber \\
%     &\leq \left| \|\left(A(SA)^\dagger - A(S^\prime A)^\dagger \right)Sb^\perp \|_2 + \| A(S^\prime A)^\dagger Sb^\perp \|_2 - \| A(S^\prime A)^\dagger S^\prime b^\perp \|_2\right| \nonumber \\
%     &\leq \|\left(A(SA)^\dagger - A(S^\prime A)^\dagger \right)Sb^\perp \|_2 + \|A(S^\prime A)^\dagger (S-S^\prime)b^\perp \|_2 \nonumber \\
%     &\leq \|\left(A(SA)^\dagger - A(S^\prime A)^\dagger \right)Sb^\perp \|_2 + \|A(S^\prime A)^\dagger\|_F \|S-S^\prime\|_F \|b^\perp \|_2 \nonumber \\
%     &\leq \|A\|_F^2 \|SA\|_2 \|S^\prime A\|_2 \|S-S^\prime\|_F \|Sb^\perp \|_2 + \|A(S^\prime A)^\dagger\|_F \|S-S^\prime\|_F \|b^\perp \|_2 \nonumber \\
%     &= \left( \|A\|_F^2 \|SA\|_2 \|S^\prime A\|_2 \|Sb^\perp \|_2 + \|A(S^\prime A)^\dagger\|_F\|b^\perp \|_2 \right) \|S-S^\prime\|_F \nonumber \\
%     &\leq \left( \right) \|S-S^\prime\|_F
% \end{align}

% \burak{Inequality'leri yazarken absolute value'larla ilgili bir hata yapmis olabilirim, ona dikatli bakacagim tekrar}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \mert{Bu sekilde yapinca uncondition edince sorun olmamasi lazim degil mi?}

% \burak{Uncondition derken, tum $S$ matrisi uzerinden Lipschitz concentration result bulmayi diyorsunuz degil mi?}

% \mert{Evet, bu sekilde istedigimiz full expectation'dan deviate etme probabiltysini bulacagiz, ve uncondition ederek istedigimiz sonuc cikacak}

% \burak{Boyle yapinca direk olarak $P(f(\hat{x}) - f(x^*) - \Exs[f(\hat{x}) - f(x^*)] < \epsilon)$ probability'sini bulacagiz degil mi? Conditioning nereden kaynaklanacak onu tam anlamadim sanirim.}

% \mert{Evet haklisin. Benim demek istedigim, buradaki lipschitz constant $\sigma_{\min}(SU)$'ya depend edecegi icin onun icin bir conditioning gerekecek. Ama sanirim bunu yapabiliriz?}

% \burak{Evet haklisiniz, simdi anladim. Halledebiliriz belki bu durumda.}

% \mert{Ayrica, soyle bir approach daha olabilir. Bugun konustugumuz gibi $tr M^TM= \|A(SA)^{\dagger}\|_F^2$'in expectation'ina ne kadar yakin olduguna ihtiyacigimiz vardi, Gaussian quadratic concentrationi kullanirken. Sadece burasi icin de lipschitz concentration'i kullanabiliriz. $g(S) = \|A(SA)^{\dagger}\|_F$ 'in Lipschitz constantini bulabiliriz pseudo-inverse perturbation bound'u ile (e-mail'de gonderdigim). Bunu da bugun konustugumuz gibi combine edebiliriz. Ama bu approachtaki Lipschitz constanti cok kucuk cikmayabilir. Diger full Lipschitz concentration daha iyi gibi.}

% \mert{Bu arada, bize Lipschitz concentration'da $\|S-S^\prime\|_F$ cinsindein Lipschitz constanti gerekli, o yuzden pseudo-inverse perturbation resultlarinda perturbation'in Frobenius norm'u cinsinden olanlar lazim. Emailde yolladigim paperda olmasi lazim.}

% \burak{Anladim hocam tesekkurler.}

% \subsection{Trace Concentration to Fix the Conditional Expectation Problem}
% \mert{$\|A(SA)^\dagger\|_F^2=\tr (U^TS^T S U)^{-1}$'nin expectationi yakininda concentrate oldugunu gostermek icin (bunu ilk iki elde ettigimiz boundlar ile birlikte kullanip $SA$ conditional / unconditional expectation sorununu cozmek icin) su sekilde Lipschitz concentration kullanabiliriz:
% }
% \mert{$g(S) = \|A(SA)^\dagger\|_F$'in Lipschitz constanti $\|A\|_2^2\|(SA)^\dagger\|_2\|(S^\prime A)^\dagger\|_2 $ gibi bir sey cikiyor pseudo-inverse perturbation formulu ile. $S$'in $1/\sqrt{m}$ normalizasyonuna dikkat edersek, Lipschitz concentration ile 
% $$\mathbb{P} \left[ \|A(SA)^\dagger\|_F > \Exs \|A(SA)^\dagger\|_F + \epsilon  \right] \le e^{-m\epsilon^2 C} $$
% oluyor. Jensen's inequality ile $\Exs \|A(SA)^\dagger\|_F \le \sqrt{\theta_2}$, ve $\epsilon$'u $\sqrt{\theta_2}$ ile scale edersek
% $$\mathbb{P} \left[ \|A(SA)^\dagger\|_F > \sqrt{\theta_2} (1+\epsilon)  \right] \le e^{-m\epsilon^2 C\theta_2} $$
% karesini alirsak
% $$\mathbb{P} \left[ \|A(SA)^\dagger\|_F^2 > \theta_2 (1+\epsilon)  \right] \le e^{-m\epsilon^2 C\theta_2} $$
% oluyor ve eq (12) ve eq (32)'deki boundlar ile combine ettigimiz zaman, bugun farkina vardigimiz conditionining ve expectation problemini cozebiliyoruz, oyle degil mi? En azindan relative error upper tail bound'unu istedigimize yakin bir hale getirebiliyoruz sanirim.
% }


% \mert{Aslinda $g^2(S) = \|A(SA)^\dagger\|_F^2$'nin de Lipschitz olmasi lazim $g^2(S) - g^2(S^\prime ) := a^2-b^2 = (a-b)(a+b)$ seklinde yazarsak ve $a+b=\|A(SA)^\dagger\|_F+\|A(S^\prime A)^\dagger\|_F$ uzerinde minimum singular value high probability bound'unu kullanirsak. $\Exs g^2(S)=\theta_2$ oldugunu tam bildigimiz icin, iki tarafli concentration sagliyor. Bu sekilde relative error lower tail boundunu da fix edebiliriz.}



% \burak{Lipshitz constant teriminin $S$'e bagli olmasi, yani "constant" olmamasi, bir sorun yaratabilir mi acaba? Yukarda, "Lipschitz Concentration on the Full Sketching Matrix" subsectioninda, Lipschitz constanti S'in bir fonksiyonu olarak bulabiliyoruz. Bunun boyle olmasi, Lipschitz concentration bound'da bir problem yaratabilir mi diye aklima takildi.}

% \mert{S singular valuelari uzerinden bir event'e condition ettigimiz zaman olmuyor mu?}
% \burak{O sekilde conditioning yapinca, $S$ artik iid Gaussian olmayacak galiba, o yuzden Lipschitz concentration result'i direk kullanamayabiliriz.}



% \burak{Sanirim, Lipshitz concentration proof'unda Lipshitz constant kullanilan yere baksak, orada degisiklik yaparak halledebiliriz:
% \begin{align}
    % \Exs \left[e^{\lambda (f(X)-\Exs[f(X)])} \right] &\leq \Exs \left[e^{\frac{\lambda^2 \pi^2}{8} \|\nabla f(X) \|_2^2} \right] \nonumber \\
%     &\leq \Exs \left[e^{\frac{1}{8} \lambda^2\pi^2 L(S)^2}\right] \nonumber \\
%     &\leq \Exs \left[e^{\frac{1}{8} \lambda^2 \pi^2 \left(\frac{\sqrt{d} \|Sb^\perp\|_2 }{\sigma_{\min}(SU)\sigma_{\min}(S^\prime U)} + \frac{\|b^\perp\|_2}{\sigma_{\min}(S^\prime U)}  \right)^2} \right] \nonumber \\
%     &\leq \Exs \left[.. | E  \right] P(E) + \Exs \left[.. | E^C \right] P(E^C) \nonumber \\
%     &\leq \Exs \left[ e^{\frac{1}{8} \lambda^2 \pi^2 \left( \frac{\sqrt{d} \|Sb^\perp\|_2}{(1-\sqrt{d/m}+t)^2} +  \frac{\|b^\perp\|_2}{1-\sqrt{d/m}+t} \right)^2}\right] e^{-mt^2/2} + \Exs \left[ \right]
% \end{align}
% where we defined the event $E$ as $\sigma_{\min}(SU) \geq 1 - \sqrt{d/m} + t)$. We used the following probability bound:
% \begin{align}
%     P(\sigma_{\min}(SU) \geq 1 - \sqrt{d/m} + t) \leq \exp(-mt^2/2)
% \end{align}
% Bu islemlerden cok temiz bir sonuc cikmayacak gibi duruyor.
% }

% \mert{Singular value'lar uzerinden olan event'e bastan condition edip, full Lipschitz concentration'i uyguladigimiz zaman event'e conditional expectation'a concentration'unu elde edebiliyoruz degil mi?}


% \mert{Yani en basindan $\mathbb{P}(relative error > \mathbb{E} [relative error|E] +t  | \sigma_{\min}(SU)\ge 1-\epsilon)\le e^{-t^2 ...}$. Buradaki icerideki expectation singular value uzerindeki event'e conditional. Ama conditional ve unconditional expectation uzerinde bir bound var
% $$\Exs \| A(SA)^{\dagger} S b^\perp \|_2^2 = \Exs [\| A(SA)^{\dagger} S b^\perp \|_2^2|E]P(E) + \Exs [\| A(SA)^{\dagger} S b^\perp \|_2^2|E^c]P(E^c) $$
%
% O zaman $\Exs [\| A(SA)^{\dagger} S b^\perp \|_2^2|E]P(E) \le \Exs \| A(SA)^{\dagger} S b^\perp \|_2^2 $ oluyor istedigimiz sekilde?
% }
% \burak{$P(E)$ carpanindan dolayi istedigimiz seyi bulabilecek miyiz?}

% \mert{Onun $1-exp(-...)$ oldugunu biliyoruz.}

% \burak{Event'e conditioned oldugunda, $S|E$'nin distribution'u i.i.d. Gaussian oluyor mu? Olmazsa, full Lipschitz concentration bound'ini apply edemeyebiliriz? }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{New Approach for Bounding the Error Probability}
% % Let us consider the probability
% % \begin{align}
% %     P&\left(f(\hat{x}) - f(x^*) > \Exs_{Sb^\perp}[f(\hat{x}) - f(x^*)|SA] + \epsilon |SA \right)
% % \end{align}
% % where the randomness in the probability is due to $SA$ and $Sb^\perp$ and
% Th expectation of the error with respect to $Sb^\perp$ is 
% \begin{align}
%     \Exs_{Sb^\perp}[f(\hat{x}) - f(x^*)|SA] &= \Exs_{Sb^\perp} [\|(SU)^\dagger Sb^\perp\|_2^2 | SA] \nonumber \\
%     &= \frac{f(x^*)}{m} \tr \left( (U^TS^TSU)^{-1} \right)
% \end{align}
% %
% % It follows that this is equivalent to the probability
% % \begin{align}
% %      P&\left(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \tr \left( (U^TS^TSU)^{-1}\right) + \epsilon | SA \right)
% % \end{align}
% % where the randomness of the probability is due to $SA$ and $Sb^\perp$.
% %

% Taking $L = \frac{\|b^\perp\|_2}{\sqrt{m}\sigma_{\min}(SU)}$, Theorem 2.4 implies
% %
% \begin{align}
%     P&\left( \sqrt{f(\hat{x}) - f(x^*)} \geq  \Exs_{Sb^\perp}[\sqrt{f(\hat{x}) - f(x^*)}|SA] + \epsilon | SA\right) \nonumber \\
%     &\leq \exp\left(-\frac{m\epsilon^2 \sigma^2_{\min}(SU)}{2\|b^\perp\|_2^2}\right)
% \end{align}
% We take the square of the RHS inside the probability and find an upper bound for it:
% \begin{align}
%      &\Exs^2_{Sb^\perp}[\sqrt{f(\hat{x}) - f(x^*)}] + 2\epsilon \Exs_{Sb^\perp}[\sqrt{f(\hat{x}) - f(x^*)}] + \epsilon^2 \nonumber \\
%      &\leq \Exs_{Sb^\perp}[f(\hat{x}) - f(x^*)] + \epsilon \sqrt{\Exs_{Sb^\perp}[f(\hat{x}) - f(x^*)]} + \epsilon^2 \nonumber \\
%      &\leq \frac{f(x^*)}{m} \tr \left( (U^TS^TSU)^{-1} \right) + \epsilon \sqrt{\frac{f(x^*)}{m} \tr \left( (U^TS^TSU)^{-1} \right)} + \epsilon^2 \nonumber \\
%      &\leq \frac{df(x^*)}{m\sigma^2_{\min}(SU)} + \epsilon \sqrt{\frac{df(x^*)}{m\sigma^2_{\min}(SU)}} + \epsilon^2 
% \end{align}
% %
% The last inequality is due to the following upper bound on the trace term:
% \begin{align}
%     \tr \left( (U^TS^TSU)^{-1}\right) &\leq d \| (U^TS^TSU)^{-1} \|_2 \nonumber \\
%     &= \frac{d}{\sigma_{\min}(U^TS^TSU)} \nonumber \\
%     &= \frac{d}{\sigma^2_{\min}(SU)}
% \end{align}
% %
% Hence, we have
% \begin{align}
%     P&\left( f(\hat{x}) - f(x^*) \geq \frac{df(x^*)}{m\sigma^2_{\min}(SU)} + \epsilon \sqrt{\frac{df(x^*)}{m\sigma^2_{\min}(SU)}} + \epsilon^2 | SA\right) \nonumber \\
%     &\leq \exp\left(-\frac{m\epsilon^2 \sigma^2_{\min}(SU)}{2f(x^*)}\right)
% \end{align}

% Taking the expectation of both sides with respect to $SA$ gives us
% \begin{align}
%     P&\left( f(\hat{x}) - f(x^*) \geq \frac{df(x^*)}{m\sigma^2_{\min}(SU)} + \epsilon \sqrt{\frac{df(x^*)}{m\sigma^2_{\min}(SU)}} + \epsilon^2 \right) \nonumber \\
%     &\leq \Exs_{SA}\left[\exp\left(-\frac{m\epsilon^2 \sigma^2_{\min}(SU)}{2f(x^*)}\right) \right]
% \end{align}
% where the probability is with respect to $SA$ and $Sb^\perp$.

% Let us define the event $E$ as $\sigma_{\min}(SU) > 1-\sqrt{d/m}-t$. Then, 
% \begin{align}
%     P&\left( f(\hat{x}) - f(x^*) \geq \frac{df(x^*)}{m\sigma^2_{\min}(SU)} +  \sqrt{ \frac{\epsilon^2df(x^*)}{m\sigma^2_{\min}(SU)}} + \epsilon^2 \right) = \nonumber \\
%     & P\left( f(\hat{x}) - f(x^*) \geq \frac{df(x^*)}{m\sigma^2_{\min}(SU)} + \sqrt{\frac{\epsilon^2 df(x^*)}{m\sigma^2_{\min}(SU)}} + \epsilon^2 |E \right)P(E) + \nonumber \\
%     &P\left( f(\hat{x}) - f(x^*) \geq \frac{df(x^*)}{m\sigma^2_{\min}(SU)} + \sqrt{\frac{\epsilon^2 df(x^*)}{m\sigma^2_{\min}(SU)}} + \epsilon^2 |E^C \right)P(E^C)
% \end{align}
% Then, we can upper bound the conditional probability
% \begin{align}
%     P( f(\hat{x}) - f(x^*) \geq \frac{df(x^*)}{m(1-\sqrt{d/m}-t)^2} + \sqrt{\frac{\epsilon^2 df(x^*)}{m(1-\sqrt{d/m}-t)^2}} + \epsilon^2 |E )
% \end{align}






% It follows that we can find an upper bound for the following probability:
% \begin{align}
%     P&\left(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \frac{d}{\sigma^2_{\min}(SU)} + \epsilon \right)
% \end{align}

% \begin{align}
%     P&\left(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \frac{d}{\sigma^2_{\min}(SU)} + \epsilon \right) = \nonumber \\
%     &P(...|E)P(E) + P(...|E^C)P(E^C)
% \end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Concentration of the trace expression around its mean}
% \begin{lemma} %\label{lem:trace_concent}
% The trace $\tr ( (U^TS^TSU)^{-1})$ is concentrated around its mean, i.e., 
% %
% \begin{align} \label{eq:trace_concent_final}
%     &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \nonumber \\
%     &\, \leq t + \frac{\epsilon}{(1-\sqrt{d/m}-\delta)^2}\big( \frac{d}{(1-\sqrt{d/m}-\delta)^2} + \frac{md}{m-d-1} \big) \Big) \nonumber \\
%     &\geq 1 - 4\exp \left(-t^2\epsilon^2 / (16m)\right) - \exp(-m\delta^2/2) .
% \end{align}
% \end{lemma}

% \mert{Sanirim su sekilde yapabiliyoruz. Bugun gonderdigim paperdaki (https://projecteuclid.org/journals/annals-of-applied-probability/volume-19/issue-6/Concentration-of-measure-and-spectra-of-random-matrices--Applications/10.1214/08-AAP548.full) Lemma 6'yi kullanarak}
% Let $i=\sqrt{-1}$ and define $\tilde S=SU$. Then we have
% \begin{align*}
%     \mathbb{P} \Big[\Big|  \frac{1}{d} \tr (\tilde S^T\tilde S-\epsilon i I)^{-1} &- \Exs \tr \frac{1}{d} (\tilde S^T\tilde S-i\epsilon I)^{-1}  \Big| >t \Big] \le 4 e^{-md^2t^2\epsilon^2/16}
% \end{align*}
% %
% \mert{Burada probability exponentindaki $md^2$ terimi dogru mu kontrole edelim bizdeki scalinge gore. Daha sonra matrix inverse perturbation ile, su sekilde bir bound elde edebiliriz}

% \begin{align*}
%     \left | \frac{1}{d} \tr (\tilde S^T \tilde S)^{-1} - (\tilde S^T \tilde S + i \epsilon I)^{-1} \right| \le \frac{\epsilon}{\sigma_{\min}(\tilde S)^2}
% \end{align*}
% \mert{Bunu yaklasik olarak yazdim, ama dogru sekli benzer olmali (daha once pseudo-inverse perturbation resulti kullanmistik Lipschitz constant bulmak icin, aynen onu kullanabiliriz burada). Daha sonra $\mathbb{P} [ \sigma_{\min}(SU)\le \frac{1}{1-\sqrt{\frac{d}{m}}} -t ]\le e^{-m t^2/2}$ bound'i ile yukaridaki iki bound'i combine edersek}

% \begin{align*}
%     \mathbb{P} \Big[\frac{1}{d} \tr (\tilde S^T\tilde S)^{-1} \ge \Exs \tr \frac{1}{d} (\tilde S^T\tilde S)^{-1}  +\epsilon+t \Big] \le 4 e^{-md^2t^2\epsilon^2/C_1} + e^{-mt^2/C_2}
% \end{align*}
% %
% \mert{gibi bir sonuc elde ederiz. Son olarak $t=\epsilon$ set edip, $t\leftarrow t/2$ koyarak}

% \begin{align*}
%     \mathbb{P} \Big[\frac{1}{d} \tr (\tilde S^T\tilde S)^{-1} \ge \Exs \tr \frac{1}{d} (\tilde S^T\tilde S)^{-1}  + t \Big] \le 5 e^{-md^2t^4/C}
% \end{align*}

% \mert{Bunu da $SA$ conditional Lipschitz ya da quadratic form concentration'dan elde ettigimiz sonuc ile kullaninca istedigimiz relative error concentration sonucunu elde ediyoruz sanirim, dogru mu? Ayni sekilde, relative error lower bound da cikiyor mu (sol tarafa dogru olan)?}


% \mert{Bu proof calisiyor ise, random matrix theory'de kullanilan terminoloji ile yazalim. Ornegin: $m(z):=\frac{1}{d} \tr (\tilde S^T\tilde S-z I)^{-1}$ Stieltjes Transform olarak biliniyor.}


% \burak{Anladim hocam, mantikli duruyor, tesekkurler.}


% The entries of $SU$ are distributed as $\mathcal{N}(0,1/m)$. 
% \begin{IEEEproof} [Proof of Lemma \ref{lem:trace_concent}]
% % Let us define $m(z) = \frac{1}{d} \tr \left((U^TS^TSU - \epsilon i I)^{-1}\right)$. 
% We start by invoking a result on the concentration of Stieltjes transforms, namely Lemma 6 of \cite{karoui09concentration}. This implies that
% %
% \begin{align} \label{eq:stieltjes_concent}
%     P&\big(| \tr (U^TS^TSU - \epsilon i I)^{-1} -\Exs[ \tr ( U^TS^TSU - \epsilon i I)^{-1}] | > t \big) \nonumber \\
%     &\leq 4\exp \left(-t^2\epsilon^2 / (16m)\right)
% \end{align}
% %
% The matrix $U^TS^TSU$ can be written as a sum of rank-1 matrices as follows:
% \begin{align}
%     U^TS^TSU = \sum_{i=1}^m (\tilde{s}_i^TU)^T (\tilde{s}_i^TU)
% \end{align}
% where $\tilde{s}_i^T \in \mathbb{R}^{1\times n}$ is the $i$'th row of $S$. The vectors $(\tilde{s}_i^TU)^T$ are independent as required by Lemma 6 of \cite{karoui09concentration}.
%
%The entries of $(\tilde{s}_i^TU)^T$ are distributed as $\mathcal{N}(0,1/m)$, and hence the entries of $(\sqrt{m}\tilde{s}_i^TU)^T$ are distributed as $\mathcal{N}(0,1)$.
%
% \burak{Lemma 6'da, $r_i$'lerin variance'larinin scaling'inin kac olarak assume edildigi yeri bulamadim. $1$ mi olmasi gerekiyor acaba? Ona gore yazdim yukariyi.}
%
% By scaling the terms inside the probability by $m$, we obtain
% \begin{align}
%     P&\big(| \frac{1}{d} \tr ( (U^TS^TSU - \frac{\epsilon}{m} i I)^{-1}) -\Exs[ \frac{1}{d} \tr ( (U^TS^TSU - \frac{\epsilon}{m} i I)^{-1}) ] | > mt \big) \nonumber \\
%     &\leq 4\exp \left(-t^2d^2\epsilon^2 / (16m)\right)
% \end{align}
% Replacing $\epsilon \leftarrow m\epsilon$, we get
% \begin{align}
%     P&\big(| \frac{1}{d} \tr ( (U^TS^TSU - \epsilon i I)^{-1}) -\Exs[ \frac{1}{d} \tr ( (U^TS^TSU - \epsilon i I)^{-1}) ] | > mt \big) \nonumber \\
%     &\leq 4\exp \left(-t^2d^2\epsilon^2 m/ 16\right)
% \end{align}
% Then replacing $t \leftarrow t/m$, we get
% \begin{align}
%     P&\big(| \frac{1}{d} \tr ( (U^TS^TSU - \epsilon i I)^{-1}) -\Exs[ \frac{1}{d} \tr ( (U^TS^TSU - \epsilon i I)^{-1}) ] | > t \big) \nonumber \\
%     &\leq 4\exp \left(-t^2d^2\epsilon^2 / (16m)\right)
% \end{align}
%
% \burak{Variance'in scaling'ine bagli olmayabilir aslinda sanki? Scaling yapmasaydik da ust satirdaki bound'in aynisi olcakti.}
% \mert{Evet, sanirim bu sekilde. Proof'una bakarak variance scaling assumption'i var mi anlayabiliriz. Olmayabilir.}
% \mert{(64)'teki bound tam istedigimiz sekilde. Biz $\frac{f(x^*)}{m} \tr (U^TS^TSU)^{-1}$'in expectationindan farkini bound etmek istiyoruz equation (54)'te. O yuzden (64)'u $\frac{d}{m}$ ile scale edip $r\leftarrow t \frac{d}{m}$ olarak degistirirsek:
% \begin{align*}
%     &P\big(| \frac{f(x^*)}{m} \tr ( (U^TS^TSU - \epsilon i I)^{-1}) -\Exs[ \frac{f(x^*)}{m} \tr ( (U^TS^TSU - \epsilon i I)^{-1}) ] | > t f(x^*) \big) \\
%     &\leq 4\exp \left(-mt^2\epsilon^2 / 16\right)
% \end{align*}
% }
% \mert{Daha sonra inverse matrix perturbation bound'u ile istedigimiz sonucu elde edebiliyoruz gibi?}
%
% \burak{Variance scaling'i onemli degil sanirim gercekten. Evet soylediginiz sekilde oluyor gibi, detayli bakacagim.}
%
% \burak{To-do: Yukaridaki islemleri daha sonra simplify edecegim, variance scaling'i onemli olmadigi icin yukardaki birkac adim gereksiz oluyor.}
% %


% Scaling both sides inside the probability by $\frac{df(x^*)}{m}$
% \begin{align}
%     P&\big(| \frac{f(x^*)}{m} \tr ( (U^TS^TSU - \epsilon i I)^{-1}) -\Exs[ \frac{f(x^*)}{m} \tr ( (U^TS^TSU - \epsilon i I)^{-1}) ] | > \frac{tdf(x^*)}{m} \big) \nonumber \\
%     &\leq 4\exp \left(-t^2d^2\epsilon^2 / (16m)\right)
% \end{align}
% %
% Changing $t \leftarrow \frac{tm}{d}$ gives us
% \begin{align} \label{eq:trace_concentration}
%     P&\big(| \frac{f(x^*)}{m} \tr ( (U^TS^TSU - \epsilon i I)^{-1}) -\Exs[ \frac{f(x^*)}{m} \tr ( (U^TS^TSU - \epsilon i I)^{-1}) ] | > tf(x^*) \big) \nonumber \\
%     &\leq 4\exp \left(-mt^2\epsilon^2 / 16\right)
% \end{align}


% \mert{Matrix inversion lemma ile $(M-z I)^{-1} - M^{-1} = z M^{-1}(I+M^{-1}z)M^{-1}$ oluyor sanirim. $\tr (M-z I)^{-1} - \tr M^{-1} \le  d |z| \|M^{-1}\|_2^2(1+|z| \|M^{-1}\|_2)$. Burada $M$'i $d\times d$ kabul ettim. Diger pseudo-inverse perturbation bound'i daha iyi olabilir.}


% \burak{Pseudo-inverse perturbation bound derken, $|\tr(A)| \leq d\|A\|_2$ kullanarak spectral norm'a gecip, sonrasinda perturbation bound'lari kullanabiliriz. Sizin aklinizdaki fikir oyle miydi?}
% \mert{Evet}

% \burak{Tesekkurler hocam anladim.}

% \mert{Eger $z=\sqrt{-1} v$ pure imaginary olursa, $\|(M-zI)^{-1} - M^{-1}\|_2\le |z| \|(M-zI)^{-1}\|_2 \|M^{-1}\|_2$ oluyor gibi matrix inverse perturbation ile. $(M-zI)^{-1}$'nin eigenvalue'lari $\frac{1}{\lambda_k+iv}$ oldugu icin magnitude'lari $\frac{1}{\sqrt{\lambda_k^2+v^2}}$. O yuzden $\|(M-zI)^{-1}\|_2\le \|M^{-1}\|_2=\frac{1}{\lambda_{\min}}$ oluyor sanirim. Burada $M$'i psd ve eigenvalue'lari $\lambda_k$ diye kabul ettim. Bunlar dogruysa $\tr ((M-zI)^{-1} - M^{-1}) \le d \|(M-zI)^{-1} - M^{-1}\|_2\le d |z| \|M^{-1}\|_2^2$. Trace'lerin basinda $f(x^*)/m$ oldugu icin $d/m$ scalingi 1'den kucuk oldugundan sorun yaratmiyor.}



% \begin{align}
%     &\left|\frac{f(x^*)}{m} \tr ( (U^TS^TSU)^{-1}) - \frac{f(x^*)}{m} \tr ( (U^TS^TSU - \epsilon i I)^{-1})\right| \nonumber \\
%     &= \left| \frac{f(x^*)}{m} \tr\left((U^TS^TSU)^{-1} - (U^TS^TSU - \epsilon i I)^{-1} \right) \right| \nonumber \\
%     &\leq \frac{df(x^*)}{m} \left\Vert (U^TS^TSU)^{-1} - (U^TS^TSU - \epsilon i I)^{-1} \right\Vert_2
% \end{align}

% \textbf{Inverse perturbation bound -- will remove this --} 
% \begin{align}
%     &\left\Vert (U^TS^TSU)^{-1} - (U^TS^TSU - \epsilon i I)^{-1} \right\Vert_2 \nonumber \\
%     &\leq \|(U^TS^TSU)^{-1}\|_2 \|(U^TS^TSU - \epsilon i I)^{-1} \|_2 \|\epsilon i I \|_2 \nonumber \\
%     &= \frac{\epsilon}{\sigma^2_{\min}(SU)}  \|(U^TS^TSU - \epsilon i I)^{-1} \|_2 \nonumber \\
%     &= \frac{\epsilon}{\sigma^2_{\min}(SU)} \frac{1}{\sqrt{\sigma^4_{\min}(SU)+\epsilon^2}}
% \end{align}

% Next, we will bound the difference between the trace terms $\tr ( (U^TS^TSU)^{-1})$ and  $\tr ( (U^TS^TSU - \epsilon i I)^{-1})$. First, we let the SVD decomposition of $SU$ be $\tilde{U} \tilde{\Sigma} \tilde{V}^T$. Then, we have the following equalities:
% %
% \begin{align}
%     SU &= \tilde{U} \tilde{\Sigma} \tilde{V}^T \nonumber \\
%     U^TS^TSU &= \tilde{V} \tilde{\Sigma}^2 {\tilde{V}}^T \nonumber \\
%     (U^TS^TSU)^{-1} &= \tilde{V} \tilde{\Sigma}^{-2} {\tilde{V}}^T \nonumber \\
%     U^TS^TSU - \epsilon i I &= \tilde{V} \diag(\tilde{\sigma}_j^2-\epsilon i) {\tilde{V}}^T \nonumber \\
%     (U^TS^TSU - \epsilon i I)^{-1} &= \tilde{V} \diag\left(\frac{1}{\tilde{\sigma}_j^2-\epsilon i}\right) {\tilde{V}}^T
% \end{align}
% Using these, we can come up with an exact expression for the norm:
% \begin{align}
%     &\left\Vert (U^TS^TSU)^{-1} - (U^TS^TSU - \epsilon i I)^{-1} \right\Vert_2 \nonumber \\
%     &= \| \tilde{V} \diag\left(\frac{1}{\tilde{\sigma}_j^2} - \frac{1}{\tilde{\sigma}_j^2-\epsilon i} \right) {\tilde{V}}^T \|_2 \nonumber \\
%     &= \| \tilde{V} \diag\left( \frac{-\epsilon i}{\tilde{\sigma}_j^2(\tilde{\sigma}_j^2-\epsilon i)} \right) {\tilde{V}}^T \|_2 \nonumber \\
%     &= \frac{\epsilon}{\sigma^2_{\min}(SU)\sqrt{\sigma^4_{\min}(SU) + \epsilon^2}}
% \end{align}
% &= \sqrt{\max\left(\left|\frac{1-\sigma^4_{\max}(SU)}{\sigma^2_{\max}(SU)} \right|, \left|\frac{1-\sigma^4_{\min}(SU)}{\sigma^2_{\min}(SU)} \right|\right)^2 + \frac{1}{\epsilon^2}}
% \mert{Inverse perturbation ile elde ettigimiz $ \frac{\epsilon}{\sigma^2_{\min}(SU)} \frac{1}{\sqrt{\sigma^4_{\min}(SU)+\frac{1}{\epsilon^2}}} \le\frac{\epsilon}{\sigma^4_{\min}(SU)}$ en iyisi gibi. Fakat $\epsilon$ sifira giderken yukaridaki exact expression infinity'ye gidiyor, ama inverse perturbation bound gitmiyor? Exact olan expression dogru mu?}

% \burak{Birkac hata varmis hocam evet, simdi duzelttim. (68) ve (69) ayni cikti simdi. Perturbation bound, exact ile ayni cikiyor yani. }

% \mert{Evet, senin exact expression cok daha iyi. Bize trace'ler arasindaki fark lazim oldugu icin su sekilde kullanabiliriz: $\left|\tr (U^TS^TSU)^{-1} - \tr(U^TS^TSU - \epsilon i I)^{-1}\right|\le \tr \tilde{V} \diag\left( \frac{-\epsilon i}{\tilde{\sigma}_j^2(\tilde{\sigma}_j^2-\epsilon i)} \right) {\tilde{V}}^T = \tr \diag\left( \frac{-\epsilon i}{\tilde{\sigma}_j^2(\tilde{\sigma}_j^2-\epsilon i)} \right) \le \epsilon \sum_j \frac{1}{\sigma_j^4}=\epsilon \tr (U^TS^TSU)^{-2}\le  \frac{\epsilon}{\sigma_{\min}(SU)^2}\tr (U^TS^TSU)^{-1} $. O zaman $(1-\frac{\epsilon}{\sigma_{\min}^2}) (U^TS^TSU)^{-1}\le \tr(U^TS^TSU - \epsilon i I)^{-1} \le  (1+\frac{\epsilon}{\sigma_{\min}^2}) (U^TS^TSU)^{-1} $ oluyor, ya da su sekilde yazabiliriz: $(1+\frac{\epsilon}{\sigma_{\min}^2})^{-1} (U^TS^TSU - \epsilon i I)^{-1}\le \tr(U^TS^TSU)^{-1} \le  (1-\frac{\epsilon}{\sigma_{\min}^2})^{-1} (U^TS^TSU - \epsilon i I)^{-1}$. Yani relative approximation elde ettik, ve dikkat edersen $d$ faktorunu save ettik (trace'i $d\|\cdot\|_2$ ile bound etmeden). }
% \burak{Evet $d$ faktorunden kurtulabiliyoruz boyle yapinca, duzeltirim yukariyi ona gore.}

% \mert{(66) ile bu bound'i combine edebiliriz, daha sonra da (41) ile combine edebiliriz. (41)'de bir hata var konustugumuz gibi: $d/(m-d-1)$ yerine conditional meani   $f(x^*)/m\tr (U^TS^TSU)^{-1}$gelecek. (41)'in sag tarafindaki probability'yi $\sigma_{\min}$ concentration event'ine condition edip $SU$ uzerinden expectation'i alirsak $P\big(relative error > 1+d/(m-d-1)+\epsilon | \sigma_{\min}(SU)\ge 1-\sqrt{d/m}-t\big)\le ...$ haline gelecek. Son olarak $P\left(relative error > 1+d/(m-d-1)+\epsilon\right)\le ... e^{-m} + ... e^{-m}$ olarak fully unconditional hale getirecegiz.  }

% \noindent The difference between the trace terms can be bounded as follows:
% %
% \begin{align}
%     &\left|\tr ( (U^TS^TSU)^{-1}) - \tr ( (U^TS^TSU - \epsilon i I)^{-1})\right| \nonumber \\
%     &= \left| \tr\left(\tilde{V} \diag\left(\frac{1}{\tilde{\sigma}_j^2} - \frac{1}{\tilde{\sigma}_j^2-\epsilon i}\right) {\tilde{V}}^T \right) \right| \nonumber \\
%     &= \left| \sum_{j=1}^d \left(\frac{1}{\tilde{\sigma}_j^2} - \frac{1}{\tilde{\sigma}_j^2-\epsilon i}\right) \right| = \left| \sum_{j=1}^d \left( \frac{-\epsilon i}{\tilde{\sigma}_j^2 (\tilde{\sigma}_j^2-\epsilon i)}\right) \right| \nonumber \\
%     &\leq \sum_{j=1}^d \left| \frac{-\epsilon i}{\tilde{\sigma}_j^2 (\tilde{\sigma}_j^2-\epsilon i)} \right| = \sum_{j=1}^d \frac{\epsilon }{\tilde{\sigma}_j^2 |\tilde{\sigma}_j^2-\epsilon i|}  \nonumber \\
%     &\leq \sum_{j=1}^d \frac{\epsilon}{\tilde{\sigma}_j^4} \leq  \sum_{j=1}^d \frac{\epsilon}{\tilde{\sigma}_j^2 \sigma^2_{\min}(SU)} \nonumber \\
%     &= \frac{\epsilon}{\sigma^2_{\min}(SU)} \sum_{j=1}^d \frac{1}{\tilde{\sigma}_j^2} = \frac{\epsilon}{\sigma^2_{\min}(SU)} \tr\left((U^TS^TSU)^{-1} \right)
% \end{align}
% %
% Equivalently, we have
% %
% \begin{align} \label{eq:trace_sandwich}
%     &\big(1-\frac{\epsilon}{\sigma^2_{\min}(SU)}\big) \tr((U^TS^TSU)^{-1}) \leq \tr ( (U^TS^TSU - \epsilon i I)^{-1}) \nonumber \\
%     &\leq \big(1+\frac{\epsilon}{\sigma^2_{\min}(SU)}\big) \tr((U^TS^TSU)^{-1})
% \end{align}
%
% \noindent Next, we combine the above result with \eqref{eq:trace_concentration}:
% \begin{align}
%     P&\big( (1-\frac{\epsilon}{\sigma^2_{\min}(SU)}) \tr ( (U^TS^TSU)^{-1}) \nonumber \\ 
%     &\quad\quad > \Exs[ (1+\frac{\epsilon}{\sigma^2_{\min}(SU)}) \tr ( (U^TS^TSU)^{-1}) ] + \frac{t}{m} \big) \nonumber \\
%     &\leq 4\exp \left(-mt^2\epsilon^2 / 16\right)
% \end{align}
% Equivalently, we have
% \begin{align}
%     P&\big( (1-\frac{\epsilon}{\sigma^2_{\min}(SU)}) \tr ( (U^TS^TSU)^{-1}) \nonumber \\ 
%     &\quad\quad > \Exs[ (1-\frac{\epsilon}{\sigma^2_{\min}(SU)}) \tr ( (U^TS^TSU)^{-1}) ] + 2\epsilon \gamma + \frac{t}{m} \big) \nonumber \\
%     &\leq 4\exp \left(-mt^2\epsilon^2 / 16\right)
% \end{align}
% where $\gamma = \Exs[\frac{\tr ( (U^TS^TSU)^{-1})}{\sigma^2_{\min}(SU)}]$
%
% \noindent \textbf{Upper bounding $\gamma$:} 
% \begin{align}
%     \gamma &= \Exs\left[\frac{\tr ( (U^TS^TSU)^{-1})}{\sigma^2_{\min}(SU)}\right] \nonumber \\
%     &= \Exs \left[ \frac{\sum_{j=1}^d \tilde{\sigma}^{-2}_j}{\sigma^2_{\min}(SU)} \right] \nonumber \\
%     &\leq \Exs\left[ \frac{d \sigma^{-2}_{\min}(SU)}{\sigma^2_{\min}(SU)} \right] = d\Exs[\sigma^{-4}_{\min}(SU)] \nonumber \\
%     &= 
% \end{align}
%
% \mert{$\sigma_{\min}(SU)$ uzerinden expectation almak yerine soyle yapsak: $E$ eventini $|\sigma_{min}(SU)-(1-\sqrt{\frac{d}{m}})|\le t$ olarak tanimlayalim. Bu eventin probabilitysi $1-2e^{-mt^2 C}$. O zaman (72)'yi condition edip yazabiliriz: $\sigma_{\min}(SU)$ yerine $(1-\sqrt{\frac{d}{m}})\pm t$ koyarak. Bu event'i uncondition edebiliriz high probability oldugu icin yani $P(..)=P(..| E)P(E) + P(.. |E^c)P(E^c)\le P(..| E)P(E) + P(E^c)$. Boylece $\sigma_{\min}$ den kurtulmus oluyoruz, yerine expectation'i $\pm t$ geliyor. Diger turlu yukarida $\gamma$'da gelen $d$ faktoru pek iyi degil. Dogru mu dedigim yontem?
% }
%
% \burak{(72)'yi condition edersek, probability'nin icindeki RHS'daki expectation degismeyecek ama degil mi? O expectation'i yine hesaplamamiz veya boundlamamiz lazim galiba? O kisimdan dolayi $d$ faktoru gelecek sanirim yine.}

% \mert{Hayir bence sorun yok. }

% \burak{Probability'nin conditioning'i expectation'da bir seyi degistirmemeli degil mi veya ben bir yeri kaciriyor olabilirim. Cunku orda expectation'in outputu deterministic bir ifade olcak, o yuzden probability'deki conditioning expectation'i degistirmeyecek diye dusundum.}

% \mert{Yukarida soyle yazmistim: $(1-\frac{\epsilon}{\sigma_{\min}^2}) (U^TS^TSU)^{-1}\le \tr(U^TS^TSU - \epsilon i I)^{-1} \le  (1+\frac{\epsilon}{\sigma_{\min}^2}) (U^TS^TSU)^{-1} $. Expectation alirsak
% $\Exs (1-\frac{\epsilon}{\sigma_{\min}^2}) (U^TS^TSU)^{-1}\le \Exs \tr(U^TS^TSU - \epsilon i I)^{-1} \le  \Exs (1+\frac{\epsilon}{\sigma_{\min}^2}) (U^TS^TSU)^{-1} $
% Bunu $\tr(U^TS^TSU)^{-1} - \Exs \tr(U^TS^TSU)^{-1}$'e uygulayinca (66)'daki concentration'in $\tr(U^TS^TSU)^{-1}$ icin hali oluyor ve bir error term geliyor. Bu error term'u $\sigma_{\min}$'e condition ederek kontrol edebiliyoruz.
% }
% \mert{Boyle yapsak da error term'de yine $d$ faktoru geliyor mu? Belki geliyordur haklisin. $d$ faktoru gelse nasil bir sonuc cikiyor en sonda?}

% \mert{(66)'yi alip, (70) ile birlestirirsek:
% \begin{align} 
%     P&\Bigg(| \frac{f(x^*)}{m} \tr ( (U^TS^TSU)^{-1}) -\Exs[ \frac{f(x^*)}{m} \tr ( (U^TS^TSU)^{-1}) |\\ &\le tf(x^*) + 2\frac{f(x^*)\epsilon}{m\sigma^2_{\min}} \tr (U^TS^TSU)^{-1} \Bigg) \nonumber \geq 1-4\exp \left(-mt^2\epsilon^2 / 16\right)
% \end{align}
% Daha sonra $\tr (U^TS^TSU)^{-1}\le d\sigma_{\min}^{-2}$'yi kullanalim. $\sigma_{\min}$ concentration'i ile birlestirirsek
% \begin{align} 
%     P&\Bigg(| \frac{f(x^*)}{m} \tr ( (U^TS^TSU)^{-1}) - \Exs[ \frac{f(x^*)}{m} \tr ( (U^TS^TSU)^{-1}) |\\ &\le tf(x^*) + 2\frac{df(x^*)\epsilon}{m(1-\sqrt{\frac{d}{m}}-\delta)^4}  \Bigg) \nonumber \geq 1-4\exp \left(-mt^2\epsilon^2 / 16\right)\\& - \exp\left(-m\delta^2/2\right)
% \end{align}
% }
% \mert{Senin buldugun (73)'ten farki aslinda sadece $ (1-\frac{\epsilon}{\sigma^2_{min}(SU)})$ carpanli olan approximation yerine dogrudan (70)'i kullanmasi. Ben bu relative carpanli olan bound'in $d$ faktorunu kurtaracagini dusunuyodum ama sanirim kurtarmiyor. Neyse ki approximationdan $d/m$ geliyor ve kucuk. Dogru mu yukaridaki bound (79)?}
% \burak{Evet sanirim dogru (79)'daki bound.}
% \mert{Ayrica (79)'daki expectation tek basina onceden alindigi icin deterministik. Conditioning altinda falan degismiyor. $\epsilon$'u scale ettikten sonra $t\leftarrow t+\epsilon$ olarak tek bir parametreye indirebiliriz. Bu sekilde en iyi relative error upper ve lower boundlari bulduktan sonra, simplify etmek icin $\delta=0.5\sqrt{d/m}$ secebiliriz. Numerik probability hesabi icin bu halini kullanmayiz ama en simple halini en basta gostermek icin cok iyi olur.}
% \burak{Anladim hocam.}


% \noindent The relations in \eqref{eq:stieltjes_concent} and \eqref{eq:trace_sandwich} together imply the following concentration result:
% %
% \begin{align}
%     &P\big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \leq t +\nonumber \\ &+\frac{\epsilon}{\sigma^2_{\min}(SU)}\left(\tr((U^TS^TSU)^{-1}) + \Exs[\tr((U^TS^TSU)^{-1})] \right) \big) \nonumber \\
%     &\geq 1 - 4\exp \left(-t^2\epsilon^2 / (16m)\right)
% \end{align}
% % \burak{66 ve 70'i birlestirince, sizin 74'te yazdiginizdan biraz farkli bir expression cikiyor sanirim: 77'de yazan expression.}

% \noindent We know that  $\Exs[\tr((U^TS^TSU)^{-1})]=\frac{md}{m-d-1}$. Also using the upper bound $\tr ((U^TS^TSU)^{-1}) \leq d\sigma_{\min}^{-2}(SU)$ yields
% \begin{align} \label{eq:trace_concent_1}
%     &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \nonumber \\
%     &\, \leq t + \frac{\epsilon}{\sigma^2_{\min}(SU)}\bigg( \frac{d}{\sigma^2_{\min}(SU)} + \frac{md}{m-d-1} \bigg) \Big) \nonumber \\
%     &\geq 1 - 4\exp \left(-t^2\epsilon^2 / (16m)\right)
% \end{align}


% The concentration inequality in \eqref{eq:trace_concent_1} and the concentration of the minimum singular value $P(\frac{1}{\sigma_{\min}(SU)} \leq \frac{1}{1-\sqrt{d/m} - \delta}) \geq 1-\exp(-m\delta^2/2)$ together imply that
% %
% \begin{align} \label{eq:trace_concent_2}
%     &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \nonumber \\
%     &\, \leq t + \frac{\epsilon}{(1-\sqrt{d/m}-\delta)^2}\big( \frac{d}{(1-\sqrt{d/m}-\delta)^2} + \frac{md}{m-d-1} \big) \Big) \nonumber \\
%     &\geq 1 - 4\exp \left(-t^2\epsilon^2 / (16m)\right) - \exp(-m\delta^2/2)
% \end{align}
% %
% This concludes the proof.



% \mert{Dogru olabilir kontrol etmedim, ama yukaridaki de neredeyse ayni sonuca gidiyor? Ekstra olan error terimi diger error terimi ile ayni orderda, oyle degil mi? Yani $\frac{f(x^*)\epsilon}{m\sigma^2_{\min}(SU)}\left(\tr((U^TS^TSU)^{-1}) + \Exs[\tr((U^TS^TSU)^{-1})\right)$ kismi order olarak $\epsilon f(x^*)\frac{d}{m}$, dogru mu?}
% \burak{Evet dogru sanirim, cok buyuk bir farkliliga yol acmayacak.}

% \burak{Simdi en kucuk singular value icin conditioning yaparsak, $\tr((U^TS^TSU)^{-1})$ terimini etkilemis oluyoruz sanki. Burdan dolayi bir problem cikiyor olabilir mi? Veya siz (75) ve (76)'daki equation'i yazarken baska bir sey mi kullandiniz?}

% \burak{Demek istedigim sey soyle aslinda: Bizim elimizde su var: $P\left(f(X) \leq g(X) + t)\right) \geq 1-a$. Burada $X$ bir random variable. $g(X)$'in de mean'i etrafinda concentrate oldugunu biliyoruz.
% \begin{align}
%     &P\left(f(X) \leq g(X) + t)\right) = \nonumber \\
%     &=P\left(f(X) \leq g(X) + t)|E\right)P(E) + P\left(f(X) \leq g(X) + t)|E^C\right)P(E^C) \nonumber \\
%     &\leq P\left(f(X) \leq s + t)|E\right)P(E) + P(E^C)
% \end{align}
% Bizim istedigimiz ifade, conditioning olmayan versiyonu: $$P(f(X)\leq s+t)$$
% Bunu elde edemiyoruz bu sekilde sanirim. 
% }


% \burak{Soyle olabilir belki: $A$ eventi $f(X) \geq g(X)+t$ olsun. $B$ eventi de $g(X) \geq s$ olsun. 
% \begin{align}
%     P(A \cap B) &= P(A) + P(B) - P(A\cup B) \nonumber \\
%     &\geq P(A) + P(B) - 1
% \end{align}
% $D$ event'i de $f(X) \geq s+t$ olsun, istedigimiz event bu olacak. Su ifade dogru sanirim: $P(D) \geq P(A \cap B)$ because every point $x$ in $A\cap B$ is also in $D$. Bu durumda soyle bir lower bound oluyor: $P(D) \geq P(A)+P(B)-1$. Ve, $P(A)$ icin lower bound zaten var. $P(B)$ icin de var.
% \begin{align}
%     P(D) \geq 1 - 4\exp \left(-mt^2\epsilon^2 / 16\right) + 1 - \exp(-m\delta^2/2) - 1
% \end{align}
% }
% \mert{Evet bu son yazdigin sekilde oluyor.}
% \burak{Event tanimlari su an biraz karisti gibi, ama benzer bir sekilde yapinca cikacak sanirim.}


% \mert{(77)'deki ilk expectation zaten deterministik, orada sorun yok. Diger expectation'i $d/\sigma_{\min}^2$ ile bound ediyoruz, ve concentration bound'i var. Bu sekilde tamam degil mi? (77)'deki ilk expectation'da mi sorun oldugunu dusunuyosun?}

% \burak{(77) ve (78)'de sorun yok sanirim. (78)'den sonra $\sigma_{\min}(SA)$'dan nasil kurtulacagimizla ilgili bir sorun var sanirim veya biseyi kaciriyor olabilirim.}

% \burak{Sizin (76)'da yazdiginiz, suna mi karsilik geliyor: $P(D) \geq P(A) - P(B)$. Bu tam dogru olmuyor galiba, bu event'lerin tanimlanma seklini goz onune alirsak. }
% \end{IEEEproof}





%%%%%%%%%%%%%%%%%%%%%
\subsection{Concentration of the error}

Before we plug the trace concentration result given in Lemma \ref{lem:trace_concent} in the concentration bound due to $Sb^\perp$, we simplify it as follows. 


% First we let $\delta=1-(k+1)\sqrt{d/m}$. Then, we note that $\frac{d}{(1-\sqrt{d/m}-\delta)^2} = \frac{d}{k^2d/m} = \frac{md}{dk^2}$. It follows that $\frac{md}{dk^2} \leq \frac{md}{m-d-1}$ for $k^2 \geq \frac{m-d-1}{d}$ and $\frac{md}{dk^2} \geq \frac{md}{m-d-1}$ for $k^2 \leq \frac{m-d-1}{d}$. This leads to the following bound:
% %
% \begin{align} \label{eq:trace_concent_3}
%     &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \nonumber \\
%     & \leq t + \epsilon \frac{2m^2d}{(m-d-1)^2} \Big) \nonumber \\
%     &\geq 1 - 4e^{-\frac{t^2\epsilon^2}{16m}} - e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}}
% \end{align}
% %
% for $k^2 \geq \frac{m-d-1}{d}$. todo: calculate for $k^2 \leq \frac{m-d-1}{d}$ ?


% \burak{Veya $\delta$'yi soyle secebiliriz: $$\delta = 1 - \sqrt{d/m} + \sqrt{\frac{1}{k-1}\frac{m-d-1}{m}}.$$ Bu durumda
% \begin{align}
%     &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \nonumber \\
%     &\, \leq t + \frac{\epsilon k(k-1)m^2d^2}{(m-d-1)^2} \Big) \nonumber \\
%     &\geq 1 - 4e^{-t^2\epsilon^2 / (16m)} - e^{-\frac{m(1 - \sqrt{d/m} + \sqrt{\frac{1}{k-1}\frac{m-d-1}{m}})^2}{2}}
% \end{align}
% } 

%%%%%
Let us pick $\delta = \sqrt{d/m}$. Then, we have
\begin{align}
    &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \nonumber \\
    &\, \leq t + \frac{\epsilon}{(1-2\sqrt{d/m})^2}\big( \frac{d}{(1-2\sqrt{d/m})^2} + \frac{md}{m-d-1} \big) \Big) \nonumber \\
    &\geq 1 - 4\exp \left(-t^2\epsilon^2 / (16m)\right) - \exp(-d/2)
\end{align}
%
We observe that
\begin{align}
    \frac{d}{(1-2\sqrt{d/m})^2} &= \frac{d}{1-4\sqrt{d/m} + 4d/m} \nonumber \\
    &= \frac{md}{m+4d-4\sqrt{md}} \nonumber \\
    &\geq \frac{md}{m-d-1}
\end{align}
for $m \geq 2d$ and $d \geq 2$.
% \begin{align}
%     \frac{md}{m-d-1} \leq \frac{md}{m-2d}
% \end{align}
% for $d \geq 1$.
%
Using this observation, we can write the following:
\begin{align}
    &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \nonumber \\
    &\, \leq t + \frac{2d\epsilon}{(1-2\sqrt{d/m})^4} \Big) \nonumber \\
    &\geq 1 - 4\exp \left(-t^2\epsilon^2 / (16m)\right) - \exp(-d/2)
\end{align}
%
We then scale $\epsilon$ by $\epsilon \leftarrow \epsilon \frac{(1-2\sqrt{d/m})^4}{2d}$ to obtain
%
\begin{align}
    &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \leq t + \epsilon \Big) \nonumber \\
    &\geq 1 - 4e^{-\frac{t^2\epsilon^2(1-2\sqrt{d/m})^8}{64md^2}} - e^{-d/2}
\end{align}
%
Letting $t=\epsilon$ and then scaling $\epsilon \leftarrow \frac{\epsilon}{2}$ give us
%
\begin{align} \label{eq:trace_concent_5}
    &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \leq \epsilon \Big) \nonumber \\
    &\geq 1 - 4e^{-\frac{\epsilon^4(1-2\sqrt{d/m})^8}{2^{10}md^2}} - e^{-d/2}
\end{align}


% We then scale $\epsilon$ by $\epsilon \leftarrow \epsilon \frac{(m-d-1)^2}{2m^2d}$:
% %
% \begin{align} \label{eq:trace_concent_4}
%     &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \leq t + \epsilon  \Big) \nonumber \\
%     &\geq 1 - 4e^{-\frac{t^2\epsilon^2(m-d-1)^4}{64m^5d^2}} - e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}}
% \end{align}
%
% Letting $t=\epsilon$ and then scaling $\epsilon \leftarrow \frac{\epsilon}{2}$ give us
% %
% \begin{align} \label{eq:trace_concent_5}
%     &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \leq \epsilon  \Big) \nonumber \\
%     &\geq 1 - 4e^{-\frac{\epsilon^4(m-d-1)^4}{2^{10}m^5d^2}} - e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}}
% \end{align}


%%%
%%%
%%%
\begin{lemma} \label{lem:gaus_quad_concent}
Concentration bound for Gaussian quadratic forms leads to
%
\begin{align} \label{eq:gaus_quad_concent}
    P&(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \tr \left( (U^TS^TSU)^{-1} \right) + \gamma | SA) \nonumber \\ 
    &\leq \exp\left(-\frac{1}{8} \frac{\gamma^2m^2}{f^2(x^*)\tr((U^TS^TSU)^{-2})} \right)
\end{align}
\end{lemma}



\begin{IEEEproof}
The proof follows from the application of the result in [cite]. Note that conditioned on $SA$, the entries of $Sb^\perp$ are i.i.d. Gaussian. Then,
%
\begin{align}
    P&(f(\hat{x}) - f(x^*) > \Exs_{Sb^\perp}[f(\hat{x})-f(x^*)] + \gamma | SA) \nonumber \\
    &=P(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \tr \left( (U^TS^TSU)^{-1} \right) + \gamma | SA) \nonumber \\ 
    &\leq \exp\left(-\frac{1}{8} \frac{\gamma^2m^2}{f^2(x^*)\tr((U^TS^TSU)^{-2})} \right)
\end{align}
This concludes the proof.
\end{IEEEproof}


Expectation of both sides of \eqref{eq:gaus_quad_concent} with respect to $SA$ yields
%
\begin{align} \label{eq:error_concent_2}
    P&(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \tr \left( (U^TS^TSU)^{-1} \right) + \gamma) \nonumber \\ 
    &\leq \Exs\left[\exp\left(-\frac{1}{8} \frac{\gamma^2m^2}{f^2(x^*)\tr((U^TS^TSU)^{-2})} \right)\right]
\end{align}
%
We can bound the right hand side using $\tr ((U^TS^TSU)^{-2}) \leq d\sigma_{\min}^{-4}(SU)$
%
\begin{align}
    \Exs&\left[\exp\left(-\frac{1}{8} \frac{\gamma^2m^2}{f^2(x^*)\tr((U^TS^TSU)^{-2})} \right)\right] \nonumber \\ 
    & \leq \Exs\left[\exp\left(-\frac{1}{8} \frac{\gamma^2m^2\sigma^4_{\min}(SU)}{df^2(x^*)} \right)\right] \nonumber \\
    &= \Exs\left[\exp\left(-\frac{1}{8} \frac{\gamma^2m^2\sigma^4_{\min}(SU)}{df^2(x^*)} \right) | E\right] P(E) \nonumber \\
    &+ \Exs\left[\exp\left(-\frac{1}{8} \frac{\gamma^2m^2\sigma^4_{\min}(SU)}{df^2(x^*)} \right) | E^C\right] P(E^C) \nonumber \\
    &\leq e^{-\frac{1}{8} \frac{\gamma^2m^2(1-\sqrt{d/m}-s)^4}{df^2(x^*)}} (1-e^{-\frac{ms^2}{2}}) + e^{-\frac{ms^2}{2}}
\end{align}
where we defined the event $E$ as $\sigma_{\min}(SU) \geq 1-\sqrt{d/m}-s$. Hence, we have
%
\begin{align} \label{eq:error_concent_3}
    P&(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \tr \left( (U^TS^TSU)^{-1} \right) + \gamma f(x^*)) \nonumber \\ 
    &\leq e^{-\frac{1}{8} \frac{\gamma^2m^2(1-\sqrt{d/m}-s)^4}{d}} (1-e^{-\frac{ms^2}{2}}) + e^{-\frac{ms^2}{2}}
\end{align}
%

We know from \eqref{eq:trace_concent_5} that $\tr((U^TS^TSU)^{-1})$ is concentrated around its mean. Hence, we obtain
%
\begin{align} \label{eq:error_concent_4}
    P&\big(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \Exs[\tr \left( (U^TS^TSU)^{-1} \right)] + \gamma f(x^*) +\frac{f(x^*)\epsilon}{m}\big) \nonumber \\
    &\leq e^{-\frac{1}{8} \frac{\gamma^2m^2(1-\sqrt{d/m}-s)^4}{d}} (1-e^{-\frac{ms^2}{2}}) + e^{-\frac{ms^2}{2}} \nonumber \\
    &\,\,+ 4e^{-\frac{\epsilon^4(1-2\sqrt{d/m})^8}{2^{10}md^2}} + e^{-d/2}
\end{align}
%
Equivalently,
%
\begin{align} \label{eq:error_concent_5}
    P&\big(f(\hat{x}) - f(x^*) > \frac{f(x^*)d}{m-d-1}  + (\gamma+\epsilon) f(x^*)\big) \nonumber \\ 
    &\leq e^{-\frac{1}{8} \frac{\gamma^2m^2(1-\sqrt{d/m}-s)^4}{d}} (1-e^{-\frac{ms^2}{2}}) + e^{-\frac{ms^2}{2}} \nonumber \\
    &\,\,+ 4e^{-\frac{\epsilon^4m^3(1-2\sqrt{d/m})^8}{2^{10}d^2}} + e^{-d/2}
\end{align}
%
Setting $\gamma=\epsilon$ and then scaling $\epsilon \leftarrow \epsilon/2$ yield
%
\begin{align} \label{eq:error_concent_6}
    P&\big(f(\hat{x}) - f(x^*) > \frac{f(x^*)d}{m-d-1}  + \epsilon f(x^*)\big) \nonumber \\ 
    &\leq e^{- \frac{\epsilon^2m^2(1-\sqrt{d/m}-s)^4}{32d}} (1-e^{-\frac{ms^2}{2}}) + e^{-\frac{ms^2}{2}} \nonumber \\
    &\,\,+ 4e^{-\frac{\epsilon^4m^3(1-2\sqrt{d/m})^8}{2^{14}d^2}} + e^{-d/2}
\end{align}

% \mert{$P(f(\hat x)/f(\hat x)>d/(m-d-1)+\epsilon)\le C_1exp(-C_2\epsilon^4 (m-d-1)^4/md^2)$ olarak exponentlari birlestirip yazalim.}


% \burak{Asagida, tum sonucu Theorem \ref{thm:concentration_single_sketch} olarak yazdim. Bu sekliyle iyi mi sizce su an?}

\noindent Let us select $s=\sqrt{d/m}$. Then, we obtain
\begin{align}
    P&\big(f(\hat{x}) - f(x^*) > \frac{f(x^*)d}{m-d-1}  + \epsilon f(x^*)\big) \nonumber \\ 
    &\leq e^{- \frac{\epsilon^2m^2(1-2\sqrt{d/m})^4}{32d}} (1-e^{-d/2}) + 4e^{-\frac{\epsilon^4m^3(1-2\sqrt{d/m})^8}{2^{14}d^2}} + 2e^{-d/2}
\end{align}
%
We observe the following
\begin{align}
    \frac{\epsilon^4m^3(1-2\sqrt{d/m})^8}{2^{14}d^2} = \frac{\epsilon^4(\sqrt{m}-2\sqrt{d})^8}{2^{14}md^2}
\end{align}
and
\begin{align}
    \frac{\epsilon^2m^2(1-2\sqrt{d/m})^4}{32d} = \frac{\epsilon^2(\sqrt{m}-2\sqrt{d})^4}{32d}
\end{align}
%
Using these observations, the bound can be more compactly written as
\begin{align} \label{eq:error_concent_7}
    P&\big(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1}  + \epsilon \big) \nonumber \\
    &\leq C_1 e^{-C_2\frac{\epsilon^2(\sqrt{m}-2\sqrt{d})^4}{md^2}\min(\epsilon^2(\sqrt{m}-2\sqrt{d})^4,md)}
\end{align}
% \burak{Single-sketch durumunda, en sade hali boyle oldu hocam, biraz karisik mi duruyor yoksa bu hali iyi mi sizce?}

% \burak{Iki regime olmasindan kurtulmak icin, proposition 1 kullanarak da yapacagim bunu, ama sanirim order olarak ayni cikacak.}


\noindent \textbf{Using Proposition 1:} The error can be expressed as:
%
\begin{align}
f(\hat{x}) - f(x^*) &= \left\Vert \frac{\|b^\perp\|_2}{\sqrt{m}} A(SA)^\dagger \frac{\sqrt{m}}{\|b^\perp\|_2} Sb^\perp \right\Vert_2^2 
\end{align}
and we define $z := \frac{\sqrt{m}}{\|b^\perp\|_2}Sb^\perp$ and $M := \frac{\|b^\perp\|_2}{\sqrt{m}} A(SA)^\dagger$. This simplifies the previous expression
\begin{align}
    f&(\hat{x}) - f(x^*) = \|Mz\|_2^2 = z^TM^TMz
\end{align}

Proposition 1 of [Concentration of quadratic forms under a Bernstein moment assumption] implies
%
\begin{align} \label{eq:prop1_singlesketch}
    &P\Big(f(\hat{x}) - f(x^*) - \Exs_{Sb^\perp}[f(\hat{x}) - f(x^*)] \nonumber \\
    &> 2\|M^TM\|_F \sqrt{\epsilon} + 2\|M^TM\|_2 \epsilon \Big| SU \Big) \leq e^{-\epsilon}
\end{align}
%
Next, we compute $\|M^TM\|_F$ and $\|M^TM\|_2$:
\begin{align}
    \|M^TM\|_F &= \frac{f(x^*)}{m} \sqrt{\tr((U^TS^TSU)^{-2})} \nonumber \\
    &\leq \frac{f(x^*)}{m} \frac{\sqrt{d}}{\sigma^2_{\min}(SU)} \\
    \|M^TM\|_2 &= \frac{f(x^*)}{m} \frac{1}{\sigma^2_{\min}(SU)}
\end{align}
%
Plugging these in \eqref{eq:prop1_singlesketch} and taking the expectation of both sides with respect to $SU$ give us
%
\begin{align}
    &P\Big(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \tr((U^TS^TSU)^{-1})\nonumber \\
    &+ 2 \frac{f(x^*)}{m\sigma^2_{\min}(SU)} ( \sqrt{\epsilon d} + \epsilon ) \Big) \leq e^{-\epsilon}
\end{align}
%
Using the trace concentration result in \eqref{eq:trace_concent_5} yields:
%
\begin{align}
    &P\Big(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \Exs[\tr((U^TS^TSU)^{-1})] \nonumber \\
    &+ 2 \frac{f(x^*)}{m\sigma^2_{\min}(SU)} ( \sqrt{\epsilon d} + \epsilon ) + \frac{f(x^*)}{m} \gamma \Big) \nonumber \\
    &\leq e^{-\epsilon} + 4e^{-\frac{\gamma^4(1-2\sqrt{d/m})^8}{2^{10}md^2}} + e^{-d/2}
\end{align}
%
Using $P(\sigma_{\min}(SU) \geq 1-\sqrt{d/m}-s) \geq 1 - e^{-ms^2/2}$, we obtain
%
\begin{align}
    &P\Big(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \Exs[\tr((U^TS^TSU)^{-1})] \nonumber \\
    &+ 2 \frac{f(x^*)}{m(1-\sqrt{d/m}-s)^2} ( \sqrt{\epsilon d} + \epsilon ) + \frac{f(x^*)}{m} \gamma \Big) \nonumber \\
    &\leq e^{-\epsilon} + 4e^{-\frac{\gamma^4(1-2\sqrt{d/m})^8}{2^{10}md^2}} + e^{-d/2} + e^{-ms^2/2}
\end{align}
%
If we let $\gamma = 2\frac{\sqrt{\epsilon d} - \epsilon}{(1-\sqrt{d/m}-s)^2}$, then we have
%
\begin{align}
    &P\Big(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \Exs[\tr((U^TS^TSU)^{-1})] \nonumber \\
    &+ 4\frac{f(x^*)}{m(1-\sqrt{d/m}-s)^2} \sqrt{\epsilon d} \Big) \nonumber \\
    &\leq e^{-\epsilon} + 4e^{-\frac{(\sqrt{\epsilon d}-\epsilon)^4(1-2\sqrt{d/m})^8}{2^{6}md^2(1-\sqrt{d/m}-s)^8}} + e^{-d/2} + e^{-ms^2/2}
\end{align}
%
If we pick $s = \sqrt{d/m}$, then
%
\begin{align}
    &P\Big(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \Exs[\tr((U^TS^TSU)^{-1})] \nonumber \\
    &+ 4\frac{f(x^*)}{m(1-2\sqrt{d/m})^2} \sqrt{\epsilon d} \Big) \nonumber \\
    &\leq e^{-\epsilon} + 4e^{-\frac{(\sqrt{\epsilon d}-\epsilon)^4}{2^{6}md^2}} + 2e^{-d/2}
\end{align}
%
Equivalently, we have
%
\begin{align}
    &P\Big(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1} + \frac{4\sqrt{\epsilon d} }{m(1-2\sqrt{d/m})^2} \Big) \nonumber \\
    &\leq e^{-\epsilon} + 4e^{-\frac{(\sqrt{\epsilon d}-\epsilon)^4}{2^{6}md^2}} + 2e^{-d/2}
\end{align}
%
Now let us set $\epsilon \leftarrow \frac{\epsilon^2}{d}$
%
\begin{align}
    &P\Big(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1} + \frac{4\epsilon }{m(1-2\sqrt{d/m})^2} \Big) \nonumber \\
    &\leq e^{-\epsilon^2/d} + 4e^{-\frac{(\epsilon-\epsilon^2/d)^4}{2^{6}md^2}} + 2e^{-d/2}
\end{align}
%
Scaling $\epsilon \leftarrow \epsilon \frac{m(1-2\sqrt{d/m})^2}{4}$ gives us
%
\begin{align}
    &P\Big(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1} + \epsilon \Big) \nonumber \\
    &\leq e^{-\frac{\epsilon^2m^2(1-2\sqrt{d/m})^4}{16d}} + 4e^{-\frac{\big(\epsilon \frac{m(1-2\sqrt{d/m})^2}{4} - \epsilon^2 \frac{m^2(1-2\sqrt{d/m})^4}{16d} \big)^4}{2^{6}md^2}} + 2e^{-d/2}
\end{align}
%
This bound can be more compactly written as
\begin{align}
    P&\big(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1}  + \epsilon \big) \leq C_1 e^{-C_2\frac{\epsilon^8m^8 (1-2\sqrt{d/m})^{16}}{md^6}}
\end{align}


% \mert{Alternatif olarak, (51)'deki $\delta$ ve (64)'deki $s$'i kucuk bir constant secsek, ornegin $\epsilon$, daha sade bir sonuc cikabilir mi? Mesela $e^{-\epsilon^2m^2(1-\sqrt{d/m}-\epsilon)^4/d^2}+e^{-m\epsilon^2}$}

\burak{
\begin{align}
    &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \nonumber \\
    &\, \leq t + \frac{2d\epsilon}{(1-\sqrt{d/m}-\delta)^4} \Big) \nonumber \\
    &\geq 1 - 4\exp \left(-t^2\epsilon^2 / (16m)\right) - \exp(-m\delta^2/2)
\end{align}
Scaling $\epsilon \leftarrow \frac{(1-\sqrt{d/m}-\delta)^4}{2d}$ gives
\begin{align}
    &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \leq t + \epsilon \Big) \nonumber \\
    &\geq 1 - 4 e^{-\frac{t^2\epsilon^2(1-\sqrt{d/m}-\delta)^8}{64md^2}} - e^{-m\delta^2/2}
\end{align}
Setting $t=\epsilon$ and then $\epsilon \leftarrow \epsilon/2$ give us
\begin{align}
    &P\Big(| \tr ( (U^TS^TSU)^{-1}) -\Exs[ \tr ( (U^TS^TSU)^{-1}) ] | \leq \epsilon \Big) \nonumber \\
    &\geq 1 - 4 e^{-\frac{\epsilon^4(1-\sqrt{d/m}-\delta)^8}{2^{10}md^2}} - e^{-m\delta^2/2}
\end{align}
%
The above trace concentration bound, Proposition 1, and the concentration of the minimum singular value together imply that
\begin{align}
    &P\Big(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \Exs[\tr((U^TS^TSU)^{-1})] \nonumber \\
    &+ 2 \frac{f(x^*)}{m(1-\sqrt{d/m}-s)^2} ( \sqrt{\epsilon d} + \epsilon ) + \frac{f(x^*)}{m} \gamma \Big) \nonumber \\
    &\leq e^{-\epsilon} + 4 e^{-\frac{\gamma^4(1-\sqrt{d/m}-\delta)^8}{2^{10}md^2}} + e^{-m\delta^2/2} + e^{-ms^2/2}
\end{align}
%
Assuming that $\sqrt{\epsilon d} > \epsilon$, we can write:
\begin{align}
    &P\Big(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \Exs[\tr((U^TS^TSU)^{-1})] \nonumber \\
    &+ \frac{4f(x^*)\sqrt{\epsilon d}}{m(1-\sqrt{d/m}-s)^2} + \frac{f(x^*)}{m} \gamma \Big) \nonumber \\
    &\leq e^{-\epsilon} + 4 e^{-\frac{\gamma^4(1-\sqrt{d/m}-\delta)^8}{2^{10}md^2}} + e^{-m\delta^2/2} + e^{-ms^2/2}
\end{align}
%
Scaling $\epsilon \leftarrow \epsilon^2/d$ yields:
\begin{align}
    &P\Big(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \Exs[\tr((U^TS^TSU)^{-1})] \nonumber \\
    &+ \frac{4f(x^*)\epsilon}{m(1-\sqrt{d/m}-s)^2} + \frac{f(x^*)}{m} \gamma \Big) \nonumber \\
    &\leq e^{-\epsilon^2/d} + 4 e^{-\frac{\gamma^4(1-\sqrt{d/m}-\delta)^8}{2^{10}md^2}} + e^{-m\delta^2/2} + e^{-ms^2/2}
\end{align}
Scaling $\epsilon \leftarrow \epsilon \frac{(1-\sqrt{d/m}-s)^2}{4}$ yields:
\begin{align}
    &P\Big(f(\hat{x}) - f(x^*) > \frac{f(x^*)}{m} \Exs[\tr((U^TS^TSU)^{-1})] + \frac{f(x^*)(\epsilon + \gamma)}{m}  \Big) \nonumber \\
    &\leq e^{-\frac{\epsilon^2(1-\sqrt{d/m}-s)^4}{16d}} + 4 e^{-\frac{\gamma^4(1-\sqrt{d/m}-\delta)^8}{2^{10}md^2}} + e^{-m\delta^2/2} + e^{-ms^2/2}
\end{align}
Letting $\gamma = \epsilon$, and scaling $\epsilon \leftarrow \epsilon m/2$ lead to
\begin{align}
    &P\big(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1}  + \epsilon \big) \nonumber \\
    &\leq e^{-\frac{\epsilon^2m^2(1-\sqrt{d/m}-s)^4}{64d}} + 4 e^{-\frac{\epsilon^4m^4(1-\sqrt{d/m}-\delta)^8}{2^{14}md^2}} + e^{-m\delta^2/2} + e^{-ms^2/2}
\end{align}
Letting $s=\delta$ leads to
\begin{align}
    &P\big(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1}  + \epsilon \big) \nonumber \\
    &\leq C_1 e^{-C_2\frac{\epsilon^2m^2(1-\sqrt{d/m}-\delta)^4}{d}\min(1, \frac{\epsilon^2m^2(1-\sqrt{d/m}-\delta)^4}{md})} + 2e^{-m\delta^2/2}
\end{align}
}


% \burak{Proposition 1'i kullanarak yapinca (82) cikiyor ve Gaussian quadratic form result'i kullanarak yapinca (68) cikiyor. (68)'de iki tane farkli regime olmasindan dolayi bir problem var.}

% \mert{Tesekkurler Burak. Bir sorum var: (68)'deki $\sqrt{m}-2\sqrt{d}$'deki $2$'yi kurtarabilir miyiz? Ornegin $\sqrt{m}-\sqrt{d}$ ya da $\sqrt{m}-(1+\epsilon)\sqrt{d}$ gibi olabilir mi?}


% \burak{$\sqrt{m}-\sqrt{d}-\delta$ gibi olabilir, veya sizin ikinci yazdiginiz gibi de olabilir. Yukardaki (85)'i devam ettirirsek oyle bir sonuc elde edebiliriz. }

% \burak{Devam ettirince (91)'deki bound cikiyor.}
% \mert{Tesekkurler. $\delta$'yi sifir secebiliyor muyuz? Bir sekilde sifir olamamasi lazim sanki?}

% \burak{Secemiyoruz evet hocam, aslinda $+e^{-m\delta^2/2}$ terimi de oluyor, (91)'e ekledim onu simdi. $\delta = \epsilon$ secip sadelestirebiliriz veya $\delta=\sqrt{d/m}$ secebiliriz.}

\mert{Tesekkurler Burak. (91)'in formu iyi. Proof'ta en son (91)'i elde edelim, ve sonra  $\asymp$ notationi kullanarak simplify edelim. Eger $c_1 d\le m \le c_2 d $ olursa (buna $m\asymp$ d deniyor) $m/d$ orani constant oluyor ve (91)'deki butun exponentlar constant$\times d$ oluyor. Su sekilde yazabiliriz: Under our assumption $m \asymp d$, the above probability is bounded by $C_1^\prime e^{-C_2^\prime m}$. Main paperda verdigimiz sonuc da bu sadelesmis hali olsun.
Bu $\asymp$ notasyonunu notations sectioninda su sekilde tanimlayabiliriz: We use the notation $m \asymp d$ for two numbers $m,d$ when there exists positive constants $c_1,c_2$ such that $c_1 d \le m \le c_2 d$. Bu yaygin bir notasyon ornegin: \href{https://math.stackexchange.com/questions/764897/what-does-this-asymp-symbol-mean-subject-analytic-number-theory}{https://math.stackexchange.com/questions/764897/what-does-this-asymp-symbol-mean-subject-analytic-number-theory}
\,\\
\,\\
\href{https://faculty.math.illinois.edu/~hildebr/595ama/ama-ch2.pdf}{https://faculty.math.illinois.edu/~hildebr/595ama/ama-ch2.pdf}}

\burak{Tesekkurler hocam, tamamdir oyle yazarim.}




% This can be more compactly written as
% %
% \begin{align} \label{eq:error_concent_7}
%     P&\big(\frac{f(\hat{x})}{f(x^*)} > \frac{m-1}{m-d-1}  + \epsilon \big) \leq C_1 e^{-C_2\frac{\epsilon^4(m-d-1)^4}{md^2}}
% \end{align}


\noindent \textbf{Lower bound:} We now obtain an error lower bound using mostly the same arguments that we used for the error upper bound.
%
We note that the concentration bound for Gaussian quadratic forms is two-sided [cite] and the other direction is
%
\begin{align}
    P&(f(\hat{x}) - f(x^*) < \frac{f(x^*)}{m} \tr \left( (U^TS^TSU)^{-1} \right) - \gamma f(x^*)) \nonumber \\ 
    &\leq e^{-\frac{1}{8} \frac{\gamma^2m^2(1-\sqrt{d/m}+s)^4}{d}} (1-e^{-\frac{ms^2}{2}}) + e^{-\frac{ms^2}{2}}
\end{align}
%
Using the concentration bound of $\tr((U^TS^TSU)^{-1})$ in \eqref{eq:trace_concent_5}, we obtain
%
\begin{align}
    P&\big(f(\hat{x}) - f(x^*) < \frac{f(x^*)}{m} \Exs[\tr \left( (U^TS^TSU)^{-1} \right)] - \gamma f(x^*) -\frac{f(x^*)\epsilon}{m}\big) \nonumber \\ 
    &\leq e^{-\frac{1}{8} \frac{\gamma^2m^2(1-\sqrt{d/m}+s)^4}{d}} (1-e^{-\frac{ms^2}{2}}) + e^{-\frac{ms^2}{2}} \nonumber \\
    &\,\,+ 4e^{-\frac{\epsilon^4(m-d-1)^4}{2^{10}m^5d^2}} + e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}}
\end{align}
%
Applying the same simplifications as before gives
%
\begin{align}
    P&\big(f(\hat{x}) - f(x^*) < \frac{f(x^*)d}{m-d-1}  - \epsilon f(x^*)\big) \nonumber \\ 
    &\leq e^{- \frac{\epsilon^2m^2(1-\sqrt{d/m}+s)^4}{32d}} (1-e^{-\frac{ms^2}{2}}) + e^{-\frac{ms^2}{2}} \nonumber \\
    &\,\,+ 4e^{-\frac{\epsilon^4(m-d-1)^4}{2^{14}md^2}} + e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}}
\end{align}


\begin{theorem} \label{thm:concentration_single_sketch}
The relative error for the single-sketch estimator $\hat{x}$ is concentrated around its mean as
%
\begin{align} 
    P&\big(\frac{f(\hat{x})}{f(x^*)} > 1+\frac{d}{m-d-1}  + \epsilon \big) \leq C_1 e^{-C_2\frac{\epsilon^4(m-d-1)^4}{md^2}}
\end{align}
and
\begin{align} 
    P&\big(\frac{f(\hat{x})}{f(x^*)} < 1+\frac{d}{m-d-1} - \epsilon \big) \leq C_1 e^{-C_2\frac{\epsilon^4(m-d-1)^4}{md^2}}
\end{align}
%
where $C_1,C_2$ are positive constants. 
\end{theorem}
%
% \mert{Evet, bu form cok iyi, tesekkurler! Distributed versiyonunu da yapalim, ve Fisher lower-boundlari.}


% \burak{Tamamdir hocam tesekkurler.}

% \burak{Yukardaki sonuc, "Improved Concentration Bounds for Gaussian
% Quadratic Forms" paperindaki theorem 1'i kullaniyor. Aslinda burda iki regime vardi. Bu teorem'i hatanin kucuk oldugu regime'e gore yazdim. Onun yerine, bu diger paperdaki proposition 1'le mi yapsak daha clean olur sizce: \href{https://arxiv.org/pdf/1901.08736.pdf}{https://arxiv.org/pdf/1901.08736.pdf}  Burdaki sonuc tek tarafli ama, sadece upper bound icin. }

We note that the lower and upper bounds of Theorem \ref{thm:concentration_single_sketch} can be combined into the following more compact form:
%
\begin{align}
    P&\left(\left| \frac{f(\hat{x})}{f(x^*)} - 1-\frac{d}{m-d-1}\right| > \epsilon \right) \leq 2C_1 e^{-C_2\frac{\epsilon^4(m-d-1)^4}{md^2}} .
\end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Averaged Estimator:} Now we consider the averaged estimator $\bar{x}=\frac{1}{q}\sum_{k=1}^q\hat{x}_k$.
\begin{align}
    f(\bar{x}) - f(x^*) &= \|A(\bar{x} - x^*)\|_2^2 \nonumber \\
    &= \left\Vert\frac{1}{q} \sum_{k=1}^q A(A^TS_k^TS_kA)^{-1}A^TS_k^TS_kb^\perp \right\Vert_2^2 \nonumber \\
    &= \left\Vert \frac{1}{q} \sum_{k=1}^q A (S_kA)^\dagger S_kb^\perp \right\Vert_2^2 \nonumber \\
    &= \left\Vert \frac{1}{q} \sum_{k=1}^q M_k z_k \right\Vert_2^2
\end{align}
%
where we defined
%
\begin{align}
    M_k &:= \frac{\|b^\perp\|_2}{\sqrt{m}} A(S_kA)^\dagger \\
    z_k &:= \frac{\sqrt{m}}{\|b^\perp\|_2} S_k b^\perp
\end{align}
%
We can manipulate the error expression
%
\begin{align}
    \sum_{k=1}^q M_k z_k &= \begin{bmatrix} M_1 & \dots & M_q \end{bmatrix} \begin{bmatrix} z_1 \\ \vdots \\ z_q \end{bmatrix} = M z
\end{align}
%
We note that the entries of the vector $z$ are distributed as i.i.d. standard normal. The error is equal to
%
\begin{align}
    f(\bar{x}) - f(x^*) = \frac{1}{q^2} \|Mz\|_2^2 = z^T\big(\frac{1}{q^2} M^TM\big)z
\end{align}
%
We will now find an equivalent expression for $\nu := 4\|\frac{1}{q^2} M^TM\|_F^2 = \frac{4}{q^4} \|M^TM\|_F^2$:
%
\begin{align}
    &\|M^TM\|_F^2 = \tr (M^TMM^TM) = \tr(MM^TMM^T) \nonumber \\
    &= \tr\left( \sum_{k=1}^q M_kM_k^T \sum_{l=1}^q M_lM_l^T \right) \nonumber \\
    &= \frac{f^2(x^*)}{m^2} \tr\left(\sum_{k=1}^q {(S_kU)^\dagger}^T (S_kU)^\dagger \sum_{l=1}^q {(S_lU)^\dagger}^T (S_lU)^\dagger \right) \nonumber \\
    &= \frac{f^2(x^*)}{m^2} \sum_{k=1}^q \sum_{l=1}^q \tr\left({(S_kU)^\dagger}^T (S_kU)^\dagger {(S_lU)^\dagger}^T (S_lU)^\dagger \right) \nonumber \\
    &= \frac{f^2(x^*)}{m^2} \Big(\sum_{k=1}^q \tr((U^TS_k^TS_kU)^{-2}) \nonumber \\
    &\quad + \sum_{k\neq l} \tr\left({(S_kU)^\dagger}^T (S_kU)^\dagger {(S_lU)^\dagger}^T (S_lU)^\dagger \right) \Big) \nonumber \\
    &\leq \frac{f^2(x^*)}{m^2} \Big(\sum_{k=1}^q \frac{d}{\sigma^4_{\min}(S_kU)} \nonumber \\
    &\quad + \sum_{k \neq l} \sqrt{\tr\left({(S_kU)^\dagger}^T (S_kU)^\dagger\right)} \sqrt{\tr\left({(S_lU)^\dagger}^T (S_lU)^\dagger\right)} \Big) \nonumber \\
    &= \frac{f^2(x^*)}{m^2} \Big(\sum_{k=1}^q \frac{d}{\sigma^4_{\min}(S_kU)} \nonumber \\
    &\quad + \sum_{k \neq l} \sqrt{\tr\left((U^TS_k^TS_kU)^{-1}\right)} \sqrt{\tr\left((U^TS_l^TS_lU)^{-1}\right)} \Big) \nonumber \\
    &\leq \frac{f^2(x^*)}{m^2} \Big(\sum_{k=1}^q \frac{d}{\sigma^4_{\min}(S_kU)} + \sum_{k\neq l} \frac{d}{\sigma_{\min}(S_kU) \sigma_{\min}(S_lU)} \Big)
\end{align}
%
where we have used the Cauchy-Schwarz inequality to bound the trace of the matrix product.

Next, we look at $\beta := \lambda_{\max}(\frac{1}{q^2}M^TM) = \frac{1}{q^2} \lambda_{\max}(M^TM)$:
\begin{align}
    \lambda_{\max}(M^TM) &=  \|M\|_2^2 = \|MM^T\|_2 \nonumber \\
    &= \|\sum_{k=1}^q M_kM_k^T \|_2 \nonumber \\
    &= \frac{\|b^\perp\|_2^2}{m}\left\Vert \sum_{k=1}^q {(S_kU)^\dagger}^T (S_kU)^\dagger \right\Vert_2 \nonumber \\
    &\leq \frac{\|b^\perp\|_2^2}{m} \sum_{k=1}^q \| {(S_kU)^\dagger}^T (S_kU)^\dagger \|_2 \nonumber \\
    &= \frac{\|b^\perp\|_2^2}{m} \sum_{k=1}^q \frac{1}{\sigma^2_{\min}(S_kU)}
\end{align}

Proposition 1 of [Concentration of quadratic forms under a Bernstein moment assumption] implies
%
\begin{align}
    &P\Big(f(\bar{x}) - f(x^*) - \Exs_{S_kb^\perp}[f(\bar{x}) - f(x^*)] \nonumber \\
    &> \frac{2}{q^2}\|M^TM\|_F \sqrt{\epsilon} + \frac{2}{q^2} \|M^TM\|_2 \epsilon \Big| SU_k \Big) \leq e^{-\epsilon}
\end{align}
%
We can take expectation of both sides with respect to $SU_k$, $k=1,\dots,q$ to remove the conditioning.
%
The expectation term is equal to
%
\begin{align}
    \Exs_{S_kb^\perp}[f(\bar{x}) - f(x^*)] &= \tr(\frac{1}{q^2}M^TM) = \frac{1}{q^2} \tr(MM^T) \nonumber \\
    &= \frac{f(x^*)}{mq^2} \sum_{k=1}^q \tr((U^TS_k^TS_kU)^{-1})
\end{align}
%
Hence we have
%
\begin{align}
    &P\Big(f(\bar{x}) - f(x^*) - \frac{f(x^*)}{mq^2} \sum_{k=1}^q \tr((U^TS_k^TS_kU)^{-1}) \nonumber \\
    &> \frac{2}{q^2}\|M^TM\|_F \sqrt{\epsilon} + \frac{2}{q^2} \|M^TM\|_2 \epsilon \Big) \leq e^{-\epsilon}
\end{align}
%
Using Lemma \ref{lem:trace_concent} for the concentration of the trace terms, we obtain
%
\begin{align}
    &P\Big(f(\bar{x}) - f(x^*) - \frac{f(x^*)}{mq^2} \sum_{k=1}^q \Exs[\tr((U^TS_k^TS_kU)^{-1})] \nonumber \\
    &> \frac{2}{q^2}\|M^TM\|_F \sqrt{\epsilon} + \frac{2}{q^2} \|M^TM\|_2 \epsilon + \frac{f(x^*)\gamma }{mq} \Big) \nonumber \\
    &\leq e^{-\epsilon} + q \big(4e^{-\frac{\gamma^4(m-d-1)^4}{2^{10}m^5d^2}} + e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}} \big)
\end{align}
%
Finally, we have
%
\begin{align}
    &P\Big(f(\bar{x}) - f(x^*) - \frac{f(x^*)}{mq^2} \sum_{k=1}^q \Exs[\tr((U^TS_k^TS_kU)^{-1})] \nonumber \\
    &> \frac{2f(x^*)}{mq^2}\bigg(\sqrt{\epsilon}\sqrt{\frac{qd}{(1-\sqrt{d/m}+s)^4} + \frac{(q^2-q)d}{(1-\sqrt{d/m}+s)^2}} \nonumber \\
    &+ \epsilon\frac{q}{(1-\sqrt{d/m}+s)^2} \bigg)  \ + \frac{f(x^*)\gamma }{mq} \Big) \nonumber \\
    &\leq e^{-\epsilon} + q \big(4e^{-\frac{\gamma^4(m-d-1)^4}{2^{10}m^5d^2}} + e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}} \big) + qe^{-\frac{ms^2}{2}}
\end{align}
%
We can simplify this as
\burak{Burdaki simplification'da $s$'nin $\sqrt{d/m}$'dan kucuk oldugunu assume etmistim, daha sonra $s$'yi secme seklim buna uymuyor ama, orada bir problem var galiba.}
%
\begin{align}
    &P\Big(\frac{f(\bar{x})}{f(x^*)} > 1 + \frac{d}{q(m-d-1)} + \frac{2(\sqrt{d\epsilon}+\epsilon)}{mq(1-\sqrt{d/m}+s)^2} + \frac{\gamma }{mq} \Big) \nonumber \\
    &\leq e^{-\epsilon} + q \big(4e^{-\frac{\gamma^4(m-d-1)^4}{2^{10}m^5d^2}} + e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}} \big) + qe^{-\frac{ms^2}{2}}
\end{align}
%
Let us select $s = -1+\sqrt{d/m} + \sqrt{\frac{2}{\epsilon}(\sqrt{d\epsilon} + \epsilon)}$. Then, we have
%
\begin{align}
    &P\Big(\frac{f(\bar{x})}{f(x^*)} > 1 + \frac{d}{q(m-d-1)} + \frac{\epsilon}{mq}+ \frac{\gamma }{mq} \Big) \nonumber \\
    &\leq e^{-\epsilon} + q \big(4e^{-\frac{\gamma^4(m-d-1)^4}{2^{10}m^5d^2}} + e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}} \big) \nonumber \\
    &+ qe^{-\frac{m\big(-1+\sqrt{d/m} + \sqrt{\frac{2}{\epsilon}(\sqrt{d\epsilon} + \epsilon)}\big)^2}{2}}
\end{align}
%
Scaling $\epsilon \leftarrow m\epsilon$ and $\gamma \leftarrow m\gamma$ lead to
%
\begin{align}
    &P\Big(\frac{f(\bar{x})}{f(x^*)} > 1 + \frac{d}{q(m-d-1)} + \frac{\epsilon}{q}+ \frac{\gamma }{q} \Big) \nonumber \\
    &\leq e^{-m\epsilon} + q \big(4e^{-\frac{\gamma^4(m-d-1)^4}{2^{10}md^2}} + e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}} \big) \nonumber \\
    &+ qe^{-\frac{m\big(-1+\sqrt{d/m} + \sqrt{\frac{2}{m\epsilon}(\sqrt{dm\epsilon} + m\epsilon)}\big)^2}{2}}
\end{align}
%
Setting $\epsilon \leftarrow \gamma$ and then scaling $\epsilon \leftarrow \epsilon q/2$ yield:
%
\begin{align}
    &P\Big(\frac{f(\bar{x})}{f(x^*)} > 1 + \frac{d}{q(m-d-1)} + \epsilon\Big) \nonumber \\
    &\leq e^{-\frac{mq\epsilon}{2}} + q \big(4e^{-\frac{q^4\epsilon^4(m-d-1)^4}{2^{14}md^2}} + e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}} \big) \nonumber \\
    &+ qe^{-\frac{m\big(-1+\sqrt{d/m} + \sqrt{\frac{4}{mq\epsilon}(\sqrt{dmq\epsilon/2} + mq\epsilon/2)}\big)^2}{2}}
\end{align}
%
This can be more simply expressed as:
%
\begin{align}
    &P\Big(\frac{f(\bar{x})}{f(x^*)} > 1 + \frac{d}{q(m-d-1)} + \epsilon\Big)  \leq q C_1  e^{-C_2\frac{q^4\epsilon^4(m-d-1)^4}{md^2}}
\end{align}
% \burak{Burda aslinda en dominant exponentin hangisi oldugu, parametrelerin degerine gore farklilik gosterebilir mi? Bu sekilde yapmak dogru oldu mu ben tam emin olamadim.}

% \mert{Tesekkurler, burada $\epsilon/q$ yerine $\epsilon$ koyabiliriz. Yani error probability $e^{-mq\epsilon)/2}+e^{-q^4 \epsilon^4}$ gibi daha kucuk olur. Ayrica averaged estimator relative error'in lower-bound'ini da bulabiliriz degil mi? Bunlari da $C_1,C_2$ gibi constantlar ile tek exponent ile sadelestirelim.}

% \burak{Bu bound'i bulurken \href{https://arxiv.org/pdf/1901.08736.pdf}{https://arxiv.org/pdf/1901.08736.pdf}'teki proposition 1'i kullandim. Tek tarafli concentration bound var burda, o yuzden lower-bound'i yapmadim. }
% \mert{Bu paperdaki Gaussian quadratic form ceoncentration bound'i $\xi^TA\xi$ ve $\xi^T(-A)\xi$'ya uygulanabilecegi icin aslinda iki tarafi da ayni probability ile gecerli. Yani, (86)'nin diger tarafi $P(\textrm{relative errpr}<d/(q(m-d-1)-\epsilon)\le ...$ olarak ayni probability ile gecerli olmali.}
% \burak{Tesekkurler hocam evet $A$ ile ilgili bir condition yokmus yapabiliriz soylediginiz gibi.}

% \mert{Onceki tek sketch case'inde bu paperdaki concentration'i kullanmak daha mi iyi olur daha mi kotu?}
% \burak{Sanirim benzer bir sonuc cikacak, parametrelerin order'lari ayni olacak. Ama iki ayri regime olmamasindan dolayi belki bu concentrationi kullanmak daha temiz olabilir ?}


\textbf{Lower bound:} Proposition 1 of [Concentration of quadratic forms under a Bernstein moment assumption] implies
%
\begin{align}
    &P\Big((-f(\bar{x}) + f(x^*)) - \Exs_{S_kb^\perp}[-f(\bar{x}) + f(x^*)] \nonumber \\
    &> \frac{2}{q^2}\|-M^TM\|_F \sqrt{\epsilon} + \frac{2}{q^2} \|-M^TM\|_2 \epsilon \Big| SU_k \Big) \leq e^{-\epsilon}
\end{align}
where we used $-\frac{1}{q^2}M^TM$ as the matrix in the quadratic term.
%
Equivalently, we have
\begin{align}
    &P\Big(f(\bar{x}) - f(x^*) < \Exs_{S_kb^\perp}[f(\bar{x}) - f(x^*)] \nonumber \\
    &- \frac{2}{q^2}\|-M^TM\|_F \sqrt{\epsilon} - \frac{2}{q^2} \|-M^TM\|_2 \epsilon \Big| SU_k \Big) \leq e^{-\epsilon}
\end{align}
%
Using Lemma \ref{lem:trace_concent} for the concentration of the trace terms, we obtain
%
\begin{align}
    &P\Big(f(\bar{x}) - f(x^*) < \frac{f(x^*)}{mq^2} \sum_{k=1}^q \Exs[\tr((U^TS_k^TS_kU)^{-1})] \nonumber \\
    &- \frac{2}{q^2}\|M^TM\|_F \sqrt{\epsilon} - \frac{2}{q^2} \|M^TM\|_2 \epsilon - \frac{f(x^*)\gamma }{mq} \Big) \nonumber \\
    &\leq e^{-\epsilon} + q \big(4e^{-\frac{\gamma^4(m-d-1)^4}{2^{10}m^5d^2}} + e^{-\frac{(\sqrt{m}-(k+1)\sqrt{d})^2}{2}} \big)
\end{align}
%
Applying the same simplification steps that we used for the upper bound, we obtain
%
\begin{align}
    &P\Big(\frac{f(\bar{x})}{f(x^*)} < 1 + \frac{d}{q(m-d-1)} - \epsilon\Big)  \leq q C_1  e^{-C_2\frac{q^4\epsilon^4(m-d-1)^4}{md^2}}
\end{align}




% \burak{$4e^{-\frac{\epsilon^4(m-d-1)^4}{2^{14}md^2}}$ terimindeki paydadaki constant cok yuksek cikiyor, o yuzden ornegin $m=400,d=20$ icin, probability bound, 1'den yuksek cikiyor. $m$'i cok daha buyuk secsek daha duzgun bound cikar tabi, ama $400/20$ orani iyi gibi gelmisti bana.}
% \mert{Burada $k$ nedir?}
% \burak{$k$'yi boundlari simplify etmek icin tanimlamistim, biz seciyoruz, su kosulu saglamasi lazim ama: $k^2 \geq \frac{m-d-1}{d}$. Numerik olarak baktigimda, exponential'lar arasindaki en buyuk olan $4e^{-\frac{\epsilon^4(m-d-1)^4}{2^{14}md^2}}$ oluyor.}
% \mert{Lower-bound'da elde edebiliyor muyuz? Yani $P(f(\hat x)/f(x^*)<..)<..$}
% \burak{Bunu henuz yapmadim, bakacagim.}
% \mert{Tamam, bu boundlari simulasyon ile plot etmeye gerek yok bence. Teorik bir result olarak verelim sadece.}
% \burak{Tamamdir hocam.}

\,\\
\,\\
% \textbf{Bound via matrix inversion lemma:}
% \begin{align}
%     &(U^TS^TSU)^{-1} - (U^TS^TSU - \epsilon i I)^{-1} \nonumber \\
%     &= (U^TS^TSU)^{-1} - (U^TS^TSU)^{-1} (I-\epsilon i(U^TS^TSU)^{-1})^{-1} \nonumber \\
%     &= (U^TS^TSU)^{-1} \left(I - (I-\epsilon i(U^TS^TSU)^{-1})^{-1}\right) \nonumber \\
%     &= -\epsilon i (U^TS^TSU)^{-2} (I-\epsilon i (U^TS^TSU)^{-1})^{-1} \\
%     &= -\epsilon i ( (U^TS^TSU)^2 - \epsilon i (U^TS^TSU) )^{-1}
% \end{align}
% Then, we have
% \begin{align}
%     &\left\Vert (U^TS^TSU)^{-1} - (U^TS^TSU - \epsilon i I)^{-1} \right\Vert_2 \nonumber \\
%     &\leq \epsilon \|(U^TS^TSU)^{-2}\|_2 \| (I-\epsilon i (U^TS^TSU)^{-1})^{-1} \|_2 \nonumber \\
%     &... \nonumber \\
%     &... \nonumber \\
%     &\leq \epsilon \frac{1}{\sigma^4_{\min}(SU)} \frac{1}{\sigma} 
% \end{align}







% \mert{En sondaki sonucu suradaki proposition 1'deki gibi yazalim \href{https://arxiv.org/pdf/1901.08736.pdf}{https://arxiv.org/pdf/1901.08736.pdf}. Inequality'nin sol tarafindaki conditional expectation son yaptigimiz derivasyon ile unconditional expectation'ina concentrate oluyor.  Burada inequalitynin sag tarafinda bizim notasyonla $2\|(U^TS^TSU)^{-1}\|_F$ ve $2\|(U^TS^TSU)^{-1}\|_2$ var sanirim.  $\|(U^TS^TSU)^{-1}\|^2_F\le\|(U^TS^TSU)^{-1}\|_2 \tr (U^TS^TSU)^{-1}$ oluyor ve geriye kalan $\|(U^TS^TSU)^{-1}\|_2$'nin de concentrate oldugunu biliyoruz. Bu result icin referans  \href{https://www.hse.ru/data/2016/11/24/1113029206/Concentration\%20inequalities.pdf}{Stéphane Boucheron, Gábor Lugosi, and Pascal Massart. Concentration inequalities:
% A nonasymptotic theory of independence.}. Sayfa 39 (pdf'e gore)'da Example 2.12'nin sonunda bu quadratic form concentration'in iki farkli sekilde yazimi var, bir tanesi ilk gordugumuz sekilde digeri ikincisi.}


-- UNCOMMENT/DELETE END HERE --
